SODAWideNet++: Combining Attention and Convolutions for Salient Object Detection

Salient Object Detection (SOD) has traditionally relied on feature refinement modules that utilize the features of an ImageNet pre-trained backbone. However, this approach limits the possibility of pre-training the entire network because of the distinct nature of SOD and image classification. Additionally, the architecture of these backbones originally built for Image classification is sub-optimal for a dense prediction task like SOD. To address these issues, we propose a novel encoder-decoder-style neural network called SODAWideNet++ that is designed explicitly for SOD. Inspired by the vision transformers ability to attain a global receptive field from the initial stages, we introduce the Attention Guided Long Range Feature Extraction (AGLRFE) module, which combines large dilated convolutions and self-attention. Specifically, we use attention features to guide long-range information extracted by multiple dilated convolutions, thus taking advantage of the inductive biases of a convolution operation and the input dependency brought by self-attention. In contrast to the current paradigm of ImageNet pre-training, we modify 118K annotated images from the COCO semantic segmentation dataset by binarizing the annotations to pre-train the proposed model end-to-end. Further, we supervise the background predictions along with the foreground to push our model to generate accurate saliency predictions. SODAWideNet++ performs competitively on five different datasets while only containing 35% of the trainable parameters compared to the state-of-the-art models. The code and pre-computed saliency maps are provided at https://github.com/VimsLab/SODAWideNetPlusPlus.

==> chapters/ablation.tex <==
\section{Ablation Experiments}

Through ablation experiments, we delve into the effects of the proposed design choices on the proposed model. All reported numbers are on the DUTS test split.

\subsection{SODAWideNet vs. SODAWideNet++}

We conducted a comparative analysis of SODAWideNet and SODAWideNet++ performance, evaluating both models from scratch and after pre-training on the modified COCO dataset, ensuring comparisons were made against models of similar size for consistency. SODAWideNet++ integrates the Multi-Receptive Field Feature Aggregation Module (MRFFAM) and Multi-scale Attention (MSA) into a single module, the Attention Guided Long Range Feature Extraction (AGLRFE). This integration reduced redundancy when extracting long-range features. Additionally, incorporating background supervision in SODAWideNet++ enhances its ability to distinguish between foreground and background areas, leading to more precise saliency results. Table \ref{tab:sodawidenetvssodawidenet++} illustrates the quantitative performance.

\begin{table}[h!]
    \centering
    % \begin{adjustbox}{width=0.75\linewidth}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
         \textbf{Pre-training mechanism} & \textbf{Model} & Size (in M) & \textbf{$F_{max}$} & \textbf{MAE}  \\
         \hline
         Scratch & SODAWideNet & 9.03 & 0.883 & 0.043 \\
         \hline
         Mod. COCO & SODAWideNet & 9.03 & 0.899& 0.035\\
         \hline
         Scratch & SODAWideNet++ & 6.66& 0.881 & 0.043 \\
         \hline
         Mod. COCO & SODAWideNet++ & 6.66 & 0.901 & 0.035\\
         \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{SODAWideNet vs. SODAWideNet++.}
    \label{tab:sodawidenetvssodawidenet++}
\end{table}

% \subsection{Downsampling in the neck}

% The spatial resolution of the output from the neck is essential to our network to produce accurate saliency predictions. Famous CNN architectures like ResNet tend to reduce the spatial resolution by a factor of four, whereas, in our work, we find that reducing the spatial resolution by a factor of two produces more accurate outputs. To study this effect of downsampling, we also decrease by a factor of four and illustrate the results. From the results in Table~\ref{tab:neckablation}, it is clear that our formulation favors a higher spatial resolution to extract semantic features due to being shallow and parameter-efficient. 

% \begin{table}[h!]
%     \centering
%     % \begin{adjustbox}{width=0.5\linewidth}
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%          \textbf{Neck} \textbf{$\downarrow$} & \textbf{Model} & \textbf{$F_{max}$} & \textbf{MAE}  \\
%          \hline
%          2 & SODAWideNet++ & 0.917 & 0.029 \\
%          \hline
%          4 & SODAWideNet++ & 0.905& 0.036\\
%          \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Effect of downsampling factor in the neck.}
%     \label{tab:neckablation}
% \end{table}
% \vspace{-3em}

\subsection{ImageNet vs. COCO Pre-training}

Table~\ref{tab:cocovsimagenet} compares our proposed models' performance when pre-trained on either the ImageNet or the modified COCO dataset. The results show an improvement with COCO pre-training, where the model experiences a 1.2\% increase in performance compared to ImageNet. This significant enhancement can be attributed to the fact that ImageNet pre-training tends to separate the development of the backbone and the feature refinement modules during the pre-training phase, leading to a disconnect in feature interpretation between the encoding and decoding stages when fine-tuning for SOD. Also, training the model from scratch achieves decent performance, highlighting the effectiveness of incorporating self-attention into a convolutional neural network.

% \begin{table}[h!]
%     \centering
%     \begin{adjustbox}{width=0.75\linewidth}
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%          \textbf{Pre-training mechanism} & \textbf{Model} & \textbf{$F_{max}$} & \textbf{MAE}  \\
%          \hline
%          \multirow{3}{*}{Scratch} & UNet-S & 0.836& 0.053 \\
%           & UNet-M & 0.872& 0.042 \\
%           & UNet-L & 0.890 & 0.039 \\
%          \hline
%          \multirow{3}{*}{ImageNet} & UNet-S & 0.844 & 0.050 \\
%           & UNet-M & 0.881& 0.040 \\
%           & UNet-L & 0.895& 0.037\\
%          \hline
%          \multirow{3}{*}{COCO} & UNet-S & 0.889 & 0.039 \\
%           & UNet-M & 0.901& 0.035 \\
%           & UNet-L & 0.912& 0.030\\
%          \hline
%     \end{tabular}
%     \end{adjustbox}
%     \caption{ImageNet vs. COCO vs. Training from scratch.}
%     \label{tab:cocovsimagenet}
% \end{table}

\begin{table}[h!]
    \centering
    % \begin{adjustbox}{width=0.75\linewidth}
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Pre-training mechanism} & \textbf{Model} & \textbf{$F_{max}$} & \textbf{MAE}  \\
         \hline
         Scratch & SODAWideNet++ & 0.890 & 0.039 \\
         \hline
         ImageNet & SODAWideNet++ & 0.905& 0.036\\
         \hline
         Mod. COCO & SODAWideNet++ & 0.917& 0.029\\
         \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{ImageNet vs. COCO vs. Training from scratch.}
    \label{tab:cocovsimagenet}
\end{table}



==> chapters/abstract.tex <==
\begin{abstract}
% Salient Object Detection (SOD) has traditionally relied on feature refinement modules that utilize the features of an ImageNet pre-trained backbone. However, this approach limits the possibility of pre-training the entire network because of the distinct nature of SOD and image classification. To address this, we propose a novel encoder-decoder-style neural network called SODAWideNet++ that is designed explicitly for SOD. Our approach is inspired by the vision transformers' ability to attain a global receptive field from the initial stages and their input-dependent nature. To achieve this, we introduce the Attention Guided Long Range Feature Extraction (AGLRFE) module, which combines dilated convolutions and self-attention, and through it, we intend to take advantage of the inductive biases of a convolution operation and the input-dependency brought by self-attention. Specifically, attention features guide long-range features extracted from dilated convolutions of different dilation rates to identify salient objects. In contrast to the current paradigm of ImageNet pre-training, we modify 118K annotated images from the COCO semantic segmentation dataset by binarizing the annotations to pre-train the proposed model end-to-end. SODAWideNet++ performs competitively against other state-of-the-art models on five different datasets.
Salient Object Detection (SOD) has traditionally relied on feature refinement modules that utilize the features of an ImageNet pre-trained backbone. However, this approach limits the possibility of pre-training the entire network because of the distinct nature of SOD and image classification. Additionally, the architecture of these backbones originally built for Image classification is sub-optimal for a dense prediction task like SOD. To address these issues, we propose a novel encoder-decoder-style neural network called SODAWideNet++ that is designed explicitly for SOD. Inspired by the vision transformers' ability to attain a global receptive field from the initial stages and their input-dependent nature, we introduce the Attention Guided Long Range Feature Extraction (AGLRFE) module, which combines large dilated convolutions and self-attention. Specifically, we use attention features to guide long-range information extracted by multiple dilated convolutions to identify salient objects of various sizes, thus taking advantage of the inductive biases of a convolution operation and the input dependency brought by self-attention. In contrast to the current paradigm of ImageNet pre-training, we modify 118K annotated images from the COCO semantic segmentation dataset by binarizing the annotations to pre-train the proposed model end-to-end. Further, we supervise the background predictions along with the foreground to push our model to generate accurate saliency predictions. SODAWideNet++ performs competitively against other state-of-the-art models on five different datasets.

\keywords{Salient Object Detection \and Self Attention \and Dilated Convolutions}
\end{abstract}

==> chapters/conclusion.tex <==
\section{Conclusion}

In conclusion, our SODAWideNet++ framework integrates the strengths of vision transformers and convolutional networks through the novel AGLRFE module. By using dilated convolutions paired with self-attention mechanisms, our model combines the inductive biases of convolutions and the dynamic, input-specific capabilities of attention mechanisms. This combination identifies salient objects across varied scenes and conditions. We used binarized annotations from the COCO dataset to train the model instead of traditional ImageNet pre-training. This tailored approach aligns directly with the nuances of SOD tasks, resulting in a model with competitive performance across multiple datasets. Our results demonstrate the effectiveness of our proposed pre-training approach and model design choices, where we achieve competitive performance against state-of-the-art models.


% Our work presents a novel pre-training method for Salient Object Detection. Instead of the two-step ImageNet pre-training approach, we modify the COCO semantic segmentation dataset to generate binary saliency maps, which we use to pre-train our proposed model. Our research sheds light on exploring different pre-training schemes for Salient Object Detection. Furthermore, we employ a Siamese network to extract semantically rich features from minimal pre-training data. The Siamese network allows us to see the data twice (through the augmented branch), which is essential since we pre-train on three times less data. Additionally, forcing the network to produce identical outputs for photometrically different inputs improves performance and generalization ability. Furthermore, by guiding convolution features with attention, we imbue input-reliance into the network, further enhancing its expressivity and generalization capabilities. Finally, our results demonstrate the effectiveness of our proposed pre-training approach and model design choices, where we achieve competitive performance against state-of-the-art models with significantly fewer parameters.

==> chapters/exp_and_results.tex <==
\section{Experiments and Results}

\begin{table*}[ht!]
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{|cc|ccc|ccc|ccc|}
    \hline
      Method& Params. (M)&  \multicolumn{3}{c|}{DUTS-TE~\cite{wang2017DUTS-TE}} & \multicolumn{3}{c|}{DUT-OMRON~\cite{yang2013saliencyOMRON}} & \multicolumn{3}{c|}{HKU-IS~\cite{LiYu15HKU}} \\
    \hline
     & & $F_{max}$ & MAE  & $S_{m}$ & $F_{max}$ & MAE & $S_{m}$ & 
    $F_{max}$ & MAE &  $S_{m}$  \\
    \hline
    % \multicolumn{17}{c}{Models with Pre-trained Backbone}\\
    % \midrule
    PiCANet-R$_{\text{CVPR'18}}$~\cite{liu2018picanet}&47.22&
    0.860&0.051&0.869&
    0.803&0.065&0.832&
    0.918&0.043&0.904\\
    
    BASNet$_{\text{CVPR'19}}$~\cite{qin2019basnet}&87.06&
    0.860&0.048&0.866&
    0.805&0.056&0.836&
    0.928&0.032&0.909\\
    
    F3-Net$_{\text{AAAI'20}}$~\cite{wei2020f3net} & 26.5&
    0.891&0.035&0.888&
    0.813&0.053&0.838&
     0.937&0.028&0.917\\

    LDF$_{\text{CVPR'20}}$~\cite{ldf}& 25.15&
    0.898& 0.034&0.892 & 
    0.820&0.051&0.838 & 
    0.939&0.027&0.919 \\

    PA-KRN$_{\text{AAAI'21}}$~\cite{pakrn} & 68.68&
    0.907& 0.033&0.900 &
    0.834&0.050&0.853 &
    0.943&0.027&0.923 \\
    
    VST$_{\text{ICCV'21}}$~\cite{Liu_2021_ICCV_VST} & 44.48 &
    0.890&  0.037&0.896 & 
    0.825&0.058&0.850 & 
    0.942&0.029&0.928\\

    PSG$_{\text{TIP'21}}$~\cite{yang2021progressivepsg}&25.55&
    0.886&0.036&0.883&
    0.811&0.052&0.831&
    0.938&0.027&0.919\\
    
    EnergyTransf$_{\text{NeurIPS'21}}$~\cite{jing_ebm_sod21generative}&118.96&
    0.910&0.029&0.909&
    0.839&0.050&0.858&
    0.947&0.023&0.930\\

    RCSB$_{\text{WACV'22}}$~\cite{Ke_2022_WACV_RCSB} & 27.90& 
    0.889&0.035&0.878&
    0.810&0.045&0.820&
    0.938&0.027&0.918\\
    
    CSF-R2Net$_{\text{TPAMI'22}}$~\cite{gao2020sod100kcsf}& 36.53&
    0.890&0.037&0.890&
     0.815&0.055&0.838&
    0.935&0.030&0.921\\
    
    EDNet$_{\text{TIP'22}}$~\cite{wu2022edn} & 42.85 & 
    0.895&0.035&0.892&
    0.828&0.048&0.846&
    0.941&0.026&0.924\\
    
    PGNet$_{\text{CVPR'22}}$~\cite{xie2022pyramid} & 72.70 &
    0.917&0.027&0.911&
    0.835&0.045&0.855&
    0.948&0.024&0.929\\
    
    % ICON-S$_{\text{TPAMI'22}}$~\cite{zhuge2021salienticon} & 92.40&ImageNet-22k&
    % 0.920&0.025&0.917 & 0.930&
    % 0.855&0.042&0.869& 0.897&
    % 0.951&0.022&0.935&0.965 \\
    
    % TRACER7$_{\text{AAAI'22}}$~\cite{lee2022tracer} & 66.27&ImageNet&
    % 0.927& 0.022&0.919 & 0.934&
    % 0.834&0.042&0.846 & 0.878&
    % 0.951&0.020&0.934&0.964 \\

    % RMFormer$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&ImageNet&
    % 0.931& 0.023&0.925 & 0.933&
    % 0.861&0.040&0.877 & 0.904&
    % 0.957&0.019&0.940&0.968 \\

    ICON-R$_{\text{TPAMI'22}}$~\cite{zhuge2021salienticon} & 33.09&
    0.892&0.037&0.889 & 
    0.825&0.057&0.844& 
    0.939&0.029&0.920 \\

    TRACER5$_{\text{AAAI'22}}$~\cite{lee2022tracer} & 31.30&
    0.916& 0.026&0.909 & 
    0.834&0.042&0.847 &
    0.947&0.022&0.930 \\

    \hline

    \textbf{SODAWideNet++} & \textbf{26.58}&
    \textbf{0.917}& \textbf{0.029}&\textbf{0.910} & 
    \textbf{0.848}&\textbf{0.045}&\textbf{0.868} & 
    \textbf{0.950}&\textbf{0.024}&\textbf{0.932} \\

    \textbf{SODAWideNet++M} & \textbf{6.66}&
    \textbf{0.901}& \textbf{0.035}&\textbf{0.898} & 
    \textbf{0.844}&\textbf{0.048}&\textbf{0.861} & 
    \textbf{0.949}&\textbf{0.025}&\textbf{0.932} \\

    \textbf{SODAWideNet++S} & \textbf{1.67}&
    \textbf{0.887}& \textbf{0.039}&\textbf{0.886} & 
    \textbf{0.834}&\textbf{0.051}&\textbf{0.854} & 
    \textbf{0.941}&\textbf{0.028}&\textbf{0.925}\\
    
    % \midrule
    % \bottomrule
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on DUTS-TE, DUT-OMRON, and HKU-IS datasets.}
  \label{tab:ResultsTable1}
\end{table*}

\begin{table*}[ht!]
  \centering
  \begin{adjustbox}{width=0.8\linewidth}
  \begin{tabular}{|cc|ccc|ccc|}
    \hline
      Method& Params. (M) & \multicolumn{3}{c|}{ECSSD~\cite{shi2015hierarchicalECSSD}} & \multicolumn{3}{c|}{PASCAL-S~\cite{li2014secretsPASCAL-S}}\\
    \hline
     & &
    $F_{max}$ & MAE &  $S_{m}$  &
    $F_{max}$ & MAE &  $S_{m}$ \\
    \hline
    % \multicolumn{17}{c}{Models with Pre-trained Backbone}\\
    % \midrule
    PiCANet-R$_{\text{CVPR'18}}$~\cite{liu2018picanet}&47.22&
    0.935&0.046&0.917&
    0.868&0.078&0.852\\
    
    BASNet$_{\text{CVPR'19}}$~\cite{qin2019basnet}&87.06&
    0.942&0.037&0.916&
    0.860&0.079&0.834\\
    
    F3-Net$_{\text{AAAI'20}}$~\cite{wei2020f3net} & 26.5&
     0.945&0.033&0.924&
    0.882&0.064&0.857\\

    LDF$_{\text{CVPR'20}}$~\cite{ldf} & 25.15&
    0.950&0.034&0.924 & 
    0.887&0.062&0.859\\

    PA-KRN$_{\text{AAAI'21}}$~\cite{pakrn} & 68.68&
    0.953&0.032&0.928 & 
    -&-&-\\
    
    VST$_{\text{ICCV'21}}$~\cite{Liu_2021_ICCV_VST} & 44.48 &
    0.951&0.033&0.932&
    0.890&0.062&0.871\\

    PSG$_{\text{TIP'21}}$~\cite{yang2021progressivepsg}&25.55&
    0.949&0.031&0.925&
    0.886&0.063&0.858\\
    
    EnergyTransf$_{\text{NeurIPS'21}}$~\cite{jing_ebm_sod21generative}&118.96&
    0.959&0.023&0.942&
    0.900&0.055&0.876\\

    RCSB$_{\text{WACV'22}}$~\cite{Ke_2022_WACV_RCSB} & 27.90&
    0.944&0.033&0.921&
    0.886&0.061&0.857\\
    
    CSF-R2Net$_{\text{TPAMI'22}}$~\cite{gao2020sod100kcsf}& 36.53&
    0.950&0.033&0.930&
    0.886&0.069&0.862\\
    
    EDNet$_{\text{TIP'22}}$~\cite{wu2022edn} & 42.85 &
    0.951&0.032&0.927&
    0.891&0.065&0.860\\
    
    PGNet$_{\text{CVPR'22}}$~\cite{xie2022pyramid} & 72.70 &
    0.960&0.027&0.918&
    0.904&0.056&0.874\\
    
    ICON-R$_{\text{TPAMI'22}}$~\cite{zhuge2021salienticon} & 33.09&
    0.950&0.032&0.929 &
    0.888&0.066&0.860\\
    
    TRACER5$_{\text{AAAI'22}}$~\cite{lee2022tracer} & 31.30&
    0.956&0.027&0.933 & 
    0.907&0.051&0.878\\

    % RMFormer$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&ImageNet&
    % 0.964&0.020&0.947 & 0.938&
    % -&-&-&-\\

    \hline

    \textbf{SODAWideNet++} & \textbf{26.58}&
   \textbf{ 0.957}&\textbf{0.029}&\textbf{0.935} & 
    \textbf{0.901}&\textbf{0.062}&\textbf{0.875}\\

    \textbf{SODAWideNet++M} & \textbf{6.66}&
    \textbf{0.952}&\textbf{0.033}&\textbf{0.930} & 
    \textbf{0.895}&\textbf{0.065}&\textbf{0.866}\\

    \textbf{SODAWideNet++S} & \textbf{1.67}&
    \textbf{0.946}&\textbf{0.037}&\textbf{0.923} & 
    \textbf{0.884}&\textbf{0.070}&\textbf{0.857}\\
    
    % \midrule
    % \bottomrule
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on ECSSD and PASCAL-S datasets.}
  \label{tab:ResultsTable2}
\end{table*}

\begin{figure*}[ht!]
    \centering
    \begin{tikzpicture}[
 image/.style = {text width=0.098\linewidth,
                 inner sep=0pt, outer sep=0pt},
node distance = 0mm and 0mm
                        ] 
\node [image] (frame11)
   {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/Image.png}};
\node [image,right=of frame11] (frame21) 
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/GT.png}};
\node[image,right=of frame21] (frame31)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/NSODAWideNet++.png}};
% \node[image,right=of frame31] (frame41)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/SODAWideNet++M.png}};
% \node[image,right=of frame41] (frame51)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/SODAWideNet++S.png}};
\node[image,right=of frame31] (frame41)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/TE5.png}};
\node[image,right=of frame41] (frame51)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/ICON-R.png}};
\node[image,right=of frame51] (frame61)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PGNet.png}};
\node[image,right=of frame61] (frame71)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/EDNet.png}};
\node[image,right=of frame71] (frame81)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/CSF-R2Net.png}};
\node[image,right=of frame81] (frame91)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/RCSB.png}};
\node[image,right=of frame91] (frame101)
    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/EnergyTransformer.png}};
% \node[image,right=of frame121] (frame131)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PSG.png}};
% \node[image,right=of frame131] (frame141)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/VST.png}};
% \node[image,right=of frame141] (frame151)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PA-KRN.png}};
% \node[image,right=of frame151] (frame161)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/LDF.png}};
% \node[image,right=of frame161] (frame171)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/F3Net.png}};
% \node[image,right=of frame171] (frame181)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/BASNet.png}};
% \node[image,right=of frame181] (frame191)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PiCANet-R.png}};

\node [image, below=of frame11] (frame12)
   {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/Image.png}};
\node [image,right=of frame12] (frame22) 
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/GT.png}};
\node[image,right=of frame22] (frame32)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/NSODAWideNet++.png}};
% \node[image,right=of frame32] (frame42)
%     {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/SODAWideNet++M.png}};
% \node[image,right=of frame42] (frame52)
%     {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/SODAWideNet++S.png}};
\node[image,right=of frame32] (frame42)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/TE5.png}};
\node[image,right=of frame42] (frame52)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/ICON-R.png}};
\node[image,right=of frame52] (frame62)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/PGNet.png}};
\node[image,right=of frame62] (frame72)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/EDNet.png}};
\node[image,right=of frame72] (frame82)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/CSF-R2Net.png}};
\node[image,right=of frame82] (frame92)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/RCSB.png}};
\node[image,right=of frame92] (frame102)
    {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/EnergyTransformer.png}};
% \node[image,right=of frame122] (frame132)
%     {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/PSG.png}};
% \node[image,right=of frame132] (frame142)
%     {\includegraphics[width=\linewidth]{images/sun_bdcfkkjuwwrbigee/VST.png}};

\node [image, below=of frame12] (frame13)
   {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/Image.png}};
\node [image,right=of frame13] (frame23) 
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/GT.png}};
\node[image,right=of frame23] (frame33)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/NSODAWideNet++.png}};
% \node[image,right=of frame33] (frame43)
%     {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/SODAWideNet++M.png}};
% \node[image,right=of frame43] (frame53)
%     {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/SODAWideNet++S.png}};
\node[image,right=of frame33] (frame43)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/TE5.png}};
\node[image,right=of frame43] (frame53)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/ICON-R.png}};
\node[image,right=of frame53] (frame63)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/PGNet.png}};
\node[image,right=of frame63] (frame73)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/EDNet.png}};
\node[image,right=of frame73] (frame83)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/CSF-R2Net.png}};
\node[image,right=of frame83] (frame93)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/RCSB.png}};
\node[image,right=of frame93] (frame103)
    {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/EnergyTransformer.png}};
% \node[image,right=of frame123] (frame133)
%     {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/PSG.png}};
% \node[image,right=of frame133] (frame143)
%     {\includegraphics[width=\linewidth]{images/sun_bevucrbwugxaiuco/VST.png}};

\node [image, below=of frame13] (frame14)
   {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/Image.png}};
\node [image,right=of frame14] (frame24) 
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/GT.png}};
\node[image,right=of frame24] (frame34)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/NSODAWideNet++.png}};
\node[image,right=of frame34] (frame44)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/TE5.png}};
\node[image,right=of frame44] (frame54)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/ICON-R.png}};
\node[image,right=of frame54] (frame64)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/PGNet.png}};
\node[image,right=of frame64] (frame74)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/EDNet.png}};
\node[image,right=of frame74] (frame84)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/CSF-R2Net.png}};
\node[image,right=of frame84] (frame94)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/RCSB.png}};
\node[image,right=of frame94] (frame104)
    {\includegraphics[width=\linewidth]{images/ILSVRC2013_test_00007654/EnergyTransformer.png}};

% \node[below=of frame13]{\tiny Image};
% \node[below=of frame23]{\tiny GT};
% \node[below=of frame33]{\tiny WideUNet};
% \node[below=of frame43]{\tiny RMFormer};
% \node[below=of frame53]{\tiny TRACER7};
% \node[below=of frame63]{\tiny ICON-S};
% \node[below=of frame73]{\tiny PGNet};
% \node[below=of frame83]{\tiny EDNet};
% \node[below=of frame93]{\tiny CSF-R2Net};
% \node[below=of frame103]{\tiny RCSB};
% \node[below=of frame113]{\tiny EnergyTransf};
% \node[below=of frame123]{\tiny PSG};
% \node[below=of frame133]{\tiny VST};
% \node[below=of frame143]{\tiny PA-KRN};
% \node[below=of frame153]{\tiny LDF};
% \node[below=of frame163]{\tiny F3-Net};
% \node[below=of frame173]{\tiny BASNet};
% \node[below=of frame183]{\tiny PiCANet-R};

\node[below=of frame14]{\tiny I};
\node[below=of frame24]{\tiny GT};
\node[below=of frame34]{\tiny OURS};
% \node[below=of frame43]{\tiny OURS};
% \node[below=of frame53]{\tiny OURS};
\node[below=of frame44]{\tiny \cite{lee2022tracer}};
\node[below=of frame54]{\tiny \cite{zhuge2021salienticon}};
\node[below=of frame64]{\tiny \cite{xie2022pyramid}};
\node[below=of frame74]{\tiny \cite{wu2022edn}};
\node[below=of frame84]{\tiny \cite{gao2020sod100kcsf}};
\node[below=of frame94]{\tiny \cite{Ke_2022_WACV_RCSB}};
\node[below=of frame104]{\tiny \cite{jing_ebm_sod21generative}};
% \node[below=of frame133]{\tiny \cite{yang2021progressivepsg}};
% \node[below=of frame143]{\tiny \cite{Liu_2021_ICCV_VST}};
% \node[below=of frame151]{\tiny \cite{pakrn}};
% \node[below=of frame161]{\tiny \cite{ldf}};
% \node[below=of frame171]{\tiny \cite{wei2020f3net}};
% \node[below=of frame181]{\tiny \cite{qin2019basnet}};
% \node[below=of frame191]{\tiny \cite{liu2018picanet}};

    
\end{tikzpicture}
    \caption{In the above figure, we visually compare our results against other models.}
    \label{fig:VisualResults}
\end{figure*}

\subsection{Datasets}
We pre-train our model on the modified COCO dataset of 118K annotated images and ground truth pairs. We further augment it using horizontal and vertical flipping, taking the pre-training data size to 354K images. Then, we fine-tune our model on the DUTS~\cite{wang2017DUTS-TE} dataset, containing 10,553 images for training. We augment the data using horizontal and vertical flipping to obtain a training dataset of 31,659 images. We use five datasets to evaluate the proposed model. They are DUTS-Test\cite{wang2017DUTS-TE} consisting of 5019 images, DUT-OMRON\cite{yang2013saliencyOMRON} which consists of 5168 images, HKU-IS\cite{LiYu15HKU} which consists of 4447 images, ECSSD\cite{shi2015hierarchicalECSSD} which consists of 1000 images and PASCAL-S\cite{li2014secretsPASCAL-S} dataset consisting of 850 images.

\subsection{Implementation Details}
For COCO pre-training, we train our model for 21 epochs. The LR is set at 0.001 and multiplied by 0.5 after 15 epochs. For SOD fine-tuning, we train our model for a further 11 epochs with the same LR as the COCO stage. LR is multiplied by 0.1 after five epochs. We follow the procedure used in U-Net\cite{ronneberger2015UNET} to initialize the weights of our model. Images are resized to $384 \times 384$ for training and testing. The evaluation metrics for comparing our works with prior works are the Mean Absolute Error(MAE), maximum F-measure, and the S-measure\cite{smeasure}. The lower the MAE and the higher the $F_{max}$ and $S_{m}$ scores, the better the model.

% \subsection{Evaluation Metrics}

% The evaluation metrics used for comparing our works with prior works are the Mean Absolute Error(MAE), maximum F-measure, E-measure\cite{fan2018enhancedEmeasure}, and the S-measure\cite{smeasure}.
 
% The Mean Absolute Error(MAE) is the mean of the absolute error between the predicted saliency map and the ground truth. Equation - 1 shows the formula used to compute MAE.
% \begin{equation}
%     MAE = \frac{\sum_{i=1}^{H}\sum_{j=1}^{W}|gt_{i,j} - pred_{i, j}|}{H * W}
% \end{equation}
% Precision is the ratio of true positives and the sum of true positives and false positives. Recall is the ratio of true positives to the sum of true positives and false negatives. Precision and recall values are obtained for all the images at every threshold from 0.01 to 0.99. F-measure is the weighted harmonic mean of Precision and Recall. 
% \begin{equation}
%     F-measure = \frac{(1 + \beta^{2}) \times Precision \times Recall}{\beta^{2} \times Precision + Recall}
% \end{equation}
% We report the maximum score over all the thresholds and $\beta^{2}$ is set to 0.3.

% Finally, E-measure~\cite{fan2018enhancedEmeasure} calculates the similarity between the prediction and ground truth by calculating local pixel values image-wise mean.

\subsection{Quantitative and Qualitative Results}

Tables \ref{tab:ResultsTable1} and \ref{tab:ResultsTable2} detail the quantitative performance of SODAWideNet++ compared to 14 other state-of-the-art models. Notably, on the DUTS-TE, DUT-OMRON, and HKU-IS datasets, our model excels, achieving superior scores in both $F_{max}$ and $S_{m}$, which signifies highly confident and accurate predictions. While SODAWideNet++ generally outperforms the competition, it slightly lags behind the PGNet and TRACER5 models on the ECSSD and PASCAL-S datasets. Additionally, the smaller variants of our model, SODAWideNet++M and SODAWideNet++S, also display commendable performance, proving to be competitive with larger models across various benchmarks. The visual results, as depicted in Figure \ref{fig:VisualResults}, further substantiate the robustness of SODAWideNet++ across diverse scenarios, including images with large foreground objects, scenes containing multiple objects (notably in the second and fourth rows), and environments characterized by complex backgrounds (third and fourth rows). These results highlight the model's ability to detect salient objects in challenging visual conditions.

% In scenes with similar foreground-background colors (row - 1), with numerous objects (row - 2), and on a tiny object (row - 2, 3), WideUNet excels at detecting the salient objects. More visual results will be illustrated in the supplementary materials.

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%        Method  & Size Difference & Avg $F_{max}$ & Avg $MAE$\\
%        \hline
%          RMFormer~\cite{rmformer}& -79.3\% & -1.5\% & -0.007 \\ 
%          TRACER7~\cite{lee2022tracer}& -72.7\% & -0.6\% & -0.007\\ 
%          ICON-S~\cite{zhuge2021salienticon}& -80.47\% & -0.8\%& -0.006 \\ 
%          \hline
         
%     \end{tabular}
%     \caption{Size and Performance difference with state-of-the-art models.}
%     \label{tab:sotacomp}
% \end{table}

% \begin{figure*}[ht!]
%     \centering
%     \begin{tikzpicture}[
%  image/.style = {text width=0.055\linewidth,
%                  inner sep=0pt, outer sep=0pt},
% node distance = 0mm and 0mm
%                         ] 
% \node [image] (frame11)
%    {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/Image.png}};
% \node [image,right=of frame11] (frame21) 
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/GT.png}};
% \node[image,right=of frame21] (frame31)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/Lite.png}};
% \node[image,right=of frame31] (frame41)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/RMFormer.png}};
% \node[image,right=of frame41] (frame51)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/TE7.png}};
% \node[image,right=of frame51] (frame61)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/ICON.png}};
% \node[image,right=of frame61] (frame71)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PGNet.png}};
% \node[image,right=of frame71] (frame81)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/EDNet.png}};
% \node[image,right=of frame81] (frame91)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/CSF-R2Net.png}};
% \node[image,right=of frame91] (frame101)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/RCSB.png}};
% \node[image,right=of frame101] (frame111)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/EnergyTransformer.png}};
% \node[image,right=of frame111] (frame121)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PSG.png}};
% \node[image,right=of frame121] (frame131)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/VST.png}};
% \node[image,right=of frame131] (frame141)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PA-KRN.png}};
% \node[image,right=of frame141] (frame151)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/LDF.png}};
% \node[image,right=of frame151] (frame161)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/F3Net.png}};
% \node[image,right=of frame161] (frame171)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/BASNet.png}};
% \node[image,right=of frame171] (frame181)
%     {\includegraphics[width=\linewidth]{images/sun_azynlosmnufrooxb/PiCANet-R.png}};

% \node [image, below=of frame11] (frame12)
%    {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/Image.png}};
% \node [image,right=of frame12] (frame22) 
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/GT.png}};
% \node[image,right=of frame22] (frame32)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/Lite.png}};
% \node[image,right=of frame32] (frame42)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/RMFormer.png}};
% \node[image,right=of frame42] (frame52)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/TE7.png}};
% \node[image,right=of frame52] (frame62)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/ICON.png}};
% \node[image,right=of frame62] (frame72)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/PGNet.png}};
% \node[image,right=of frame72] (frame82)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/EDNet.png}};
% \node[image,right=of frame82] (frame92)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/CSF-R2Net.png}};
% \node[image,right=of frame92] (frame102)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/RCSB.png}};
% \node[image,right=of frame102] (frame112)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/EnergyTransformer.png}};
% \node[image,right=of frame112] (frame122)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/PSG.png}};
% \node[image,right=of frame122] (frame132)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/VST.png}};
% \node[image,right=of frame132] (frame142)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/PA-KRN.png}};
% \node[image,right=of frame142] (frame152)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/LDF.png}};
% \node[image,right=of frame152] (frame162)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/F3Net.png}};
% \node[image,right=of frame162] (frame172)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/BASNet.png}};
% \node[image,right=of frame172] (frame182)
%     {\includegraphics[width=\linewidth]{images/sun_bkfxydvemqmivotk/PiCANet-R.png}};

% \node [image, below=of frame12] (frame13)
%    {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/Image.png}};
% \node [image,right=of frame13] (frame23) 
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/GT.png}};
% \node[image,right=of frame23] (frame33)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/Lite.png}};
% \node[image,right=of frame33] (frame43)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/RMFormer.png}};
% \node[image,right=of frame43] (frame53)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/TE7.png}};
% \node[image,right=of frame53] (frame63)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/ICON.png}};
% \node[image,right=of frame63] (frame73)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/PGNet.png}};
% \node[image,right=of frame73] (frame83)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/EDNet.png}};
% \node[image,right=of frame83] (frame93)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/CSF-R2Net.png}};
% \node[image,right=of frame93] (frame103)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/RCSB.png}};
% \node[image,right=of frame103] (frame113)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/EnergyTransformer.png}};
% \node[image,right=of frame113] (frame123)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/PSG.png}};
% \node[image,right=of frame123] (frame133)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/VST.png}};
% \node[image,right=of frame133] (frame143)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/PA-KRN.png}};
% \node[image,right=of frame143] (frame153)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/LDF.png}};
% \node[image,right=of frame153] (frame163)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/F3Net.png}};
% \node[image,right=of frame163] (frame173)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/BASNet.png}};
% \node[image,right=of frame173] (frame183)
%     {\includegraphics[width=\linewidth]{images/sun_bqipzdvzujqspizw/PiCANet-R.png}};

% % \node[below=of frame13]{\tiny Image};
% % \node[below=of frame23]{\tiny GT};
% % \node[below=of frame33]{\tiny WideUNet};
% % \node[below=of frame43]{\tiny RMFormer};
% % \node[below=of frame53]{\tiny TRACER7};
% % \node[below=of frame63]{\tiny ICON-S};
% % \node[below=of frame73]{\tiny PGNet};
% % \node[below=of frame83]{\tiny EDNet};
% % \node[below=of frame93]{\tiny CSF-R2Net};
% % \node[below=of frame103]{\tiny RCSB};
% % \node[below=of frame113]{\tiny EnergyTransf};
% % \node[below=of frame123]{\tiny PSG};
% % \node[below=of frame133]{\tiny VST};
% % \node[below=of frame143]{\tiny PA-KRN};
% % \node[below=of frame153]{\tiny LDF};
% % \node[below=of frame163]{\tiny F3-Net};
% % \node[below=of frame173]{\tiny BASNet};
% % \node[below=of frame183]{\tiny PiCANet-R};

% \node[below=of frame13]{\tiny I};
% \node[below=of frame23]{\tiny GT};
% \node[below=of frame33]{\tiny OURS};
% \node[below=of frame43]{\tiny \cite{rmformer}};
% \node[below=of frame53]{\tiny \cite{lee2022tracer}};
% \node[below=of frame63]{\tiny \cite{zhuge2021salienticon}};
% \node[below=of frame73]{\tiny \cite{xie2022pyramid}};
% \node[below=of frame83]{\tiny \cite{wu2022edn}};
% \node[below=of frame93]{\tiny \cite{gao2020sod100kcsf}};
% \node[below=of frame103]{\tiny \cite{Ke_2022_WACV_RCSB}};
% \node[below=of frame113]{\tiny \cite{jing_ebm_sod21generative}};
% \node[below=of frame123]{\tiny \cite{yang2021progressivepsg}};
% \node[below=of frame133]{\tiny \cite{Liu_2021_ICCV_VST}};
% \node[below=of frame143]{\tiny \cite{pakrn}};
% \node[below=of frame153]{\tiny \cite{ldf}};
% \node[below=of frame163]{\tiny \cite{wei2020f3net}};
% \node[below=of frame173]{\tiny \cite{qin2019basnet}};
% \node[below=of frame183]{\tiny \cite{liu2018picanet}};

    
% \end{tikzpicture}
%     \caption{In the above figure, we visually compare our results against 15 other state-of-the-art models.}
%     \label{fig:VisualResults}
% \end{figure*}
% \vspace{-3em}

==> chapters/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Salient Object Detection (SOD) requires identifying the most salient object from visual data. Objects that catch a viewer's immediate attention are salient. Saliency is vital for many areas of Computer Vision, including Semantic Segmentation\cite{sun2022inferring}, Person Identification~\cite{Kim_2021_CVPRpersonsearch}, etc. The first methods for SOD \cite{cheng2014globalregionbased,jiang2013saliencyregionbased2} relied on hand-crafted priors like color, contrast, etc. With the advent of Deep Learning, the emphasis has shifted towards developing Deep Learning based solutions for SOD. Specifically, Convolutional Neural Network (CNN) based approaches demonstrated superior performance to the older non-learning-based algorithms. 

% \begin{figure}
%   \centering
%   \begin{subfigure}{0.495\linewidth}
%     \includegraphics[width=\textwidth]{images/COCOImage.png}
%     \caption{}
%     \label{fig:COCO-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.495\linewidth}
%     \includegraphics[width=\textwidth]{images/COCOAnnotation.png}
%     \caption{}
%     \label{fig:COCO-b}
%   \end{subfigure}
%   \caption{(a) COCO Image with annotations overlapped. (b) We binarize these annotations to create a SOD dataset.}
%   \label{fig:COCO}
% \end{figure}

% Over the past few years, vision transformers \cite{dosovitskiy2020vit} have replaced Convolutional Neural Networks (CNN) as the new state-of-the-art models in various Computer Vision tasks. Vision Transformer's success is attributed to the ability of self-attention to model global relationships, considering their input-dependent nature. On the other hand, famous CNN architectures \cite{he2016deepresnet, simonyan2014veryvgg16, gao2019res2net} rely on convolutions that are input-agnostic. The weights of convolutional filters in CNNs are learned during the training phase and remain fixed during inference. This static nature means that the same filters are applied regardless of the input's specific characteristics, potentially leading to suboptimal feature extraction for diverse data distributions. Also, these convolutional models have a hierarchical approach to extracting global features, which involves significant downsampling of the input through pooling layers or strides in convolutional layers. Although this downsampling is crucial for achieving a broader receptive field, it significantly loses fine-grained details, which can be critical for tasks requiring high-resolution understanding. Additionally, the hierarchical structure of CNNs struggles to capture long-range dependencies within the input image, as each convolutional layer only processes information from a limited receptive field. Although deeper networks can theoretically capture broader relationships, the loss of detail due to downsampling makes this approach inefficient. Although multiple works try to address the above-discussed problems, they are computationally expensive or still follow the same architecture. For example, deformable convolutions \cite{dai2017deformable} try to increase the receptive field of a convolutional kernel such that the weights act on the most critical locations in a feature map. However, they use a convolution layer to sample these locations, and the overall process is computationally expensive. Another work \cite{ding2022scaling} increases the receptive field of individual convolutional weights at each layer but still uses the exact four times downsampling scheme used by other CNN architectures, which is a loss of essential information without significant feature extraction.

% Current SOD models typically utilize ImageNet pre-trained backbones for initial semantic feature extraction, subsequently refining these features through specialized feature-refinement modules tailored for saliency prediction. This procedure disentangles the backbone from the feature refinement modules during the pre-training phase, leading to a sub-optimal coherence between the backbone and the specialized modules. Our proposed models are developed from the ground up to address this shortcoming, allowing for pre-training the entire network simultaneously. A key aspect of our approach involves the adaptation of the COCO semantic segmentation dataset \cite{lin2014microsoftcoco} for SOD tasks. By binarizing the segmentation labels, we convert the dataset into a format conducive to saliency detection, aligning the pre-training process more closely with the model's target application. Additionally, the COCO dataset's smaller size than ImageNet allows faster prototyping of candidate architectures. 

The latest advancements in Salient Object Detection (SOD) models primarily derive from new feature refinement modules that rely on semantic features extracted using ImageNet pre-trained backbones. However, these backbones are primarily designed for image classification and do not fully meet the complex needs of SOD. SOD often involves analyzing images with multiple objects, unlike the single-object focus typical in image classification datasets. This discrepancy can result in less optimal saliency predictions. Additionally, the standard approach of only integrating the backbone with the refinement modules during the fine-tuning phase misses a critical chance to pre-train these elements together, which could enhance overall model performance. To better address these challenges, our models are designed specifically for SOD from the ground up, allowing for the entire network to be pre-trained simultaneously. A crucial part of our approach involves adapting the COCO semantic segmentation dataset \cite{lin2014microsoftcoco} for SOD purposes by binarizing its labels. This conversion makes the dataset more suitable for saliency detection and leverages COCO's relatively smaller size than ImageNet. This advantage facilitates faster prototyping and refinement of our architectural designs, aligning the pre-training process more closely with the unique requirements of SOD and improving the effectiveness of our models.

% The past few years have seen vision transformers \cite{dosovitskiy2020vit} have replaced Convolutional Neural Networks (CNN) as the new state-of-the-art models in various Computer Vision tasks. 
% Moving toward the architectural innovations that underpin our model, it is imperative to acknowledge the significant shift that has been observed from conventional Convolutional Neural Networks \cite{he2016deepresnet,simonyan2014veryvgg16} to innovative Vision Transformers (ViTs) \cite{dosovitskiy2020vit}, which have redefined performance benchmarks in various computer vision tasks. ViTs can capture global relationships within an image through self-attention, which makes them more efficient in extracting features from the input data. This is in contrast to CNNs, which are limited by their local receptive fields and insensitivity to the unique characteristics of different inputs. CNNs use a hierarchical method for global feature extraction, which involves significant downsampling of the input via pooling or convolutional strides. This approach leads to a considerable loss of detailed information, detrimental to tasks requiring high-resolution detail. 

Moving toward the architectural innovations that underpin our model, it is crucial to recognize the dramatic shift from traditional Convolutional Neural Networks \cite{he2016deepresnet,simonyan2014veryvgg16} to Vision Transformers (ViTs) \cite{dosovitskiy2020vit}, which have significantly advanced the benchmarks across various computer vision tasks. Unlike CNNs, which are constrained by their local receptive fields and often fail to adapt to the unique characteristics of different inputs, ViTs excel by capturing global relationships and specific details within an image through self-attention. This ability enables them to extract features more effectively and precisely. CNNs typically employ a hierarchical approach to feature extraction that relies heavily on downsampling the input through methods like pooling or convolutional strides. While broadening the receptive field, this process results in a substantial loss of detail, a critical drawback for tasks requiring high-resolution outputs. Additionally, the convolution operations in CNNs are designed to detect common patterns across different instances, which does not suffice for capturing attributes unique to individual instances. Several studies have attempted to overcome these limitations but often incur high computational costs or adhere closely to conventional architectural paradigms. For example, deformable convolutions \cite{dai2017deformable} expand the receptive field adaptively to focus on the most salient regions within a feature map. However, this process remains computationally intensive due to its reliance on additional convolutional operations for sampling spatial locations. Similarly, another work \cite{ding2022scaling} proposes enhancing the receptive field at each convolutional layer. However, they continue with the standard practice of significant downsampling before substantial feature extraction, which inevitably sacrifices critical information.


% The prowess of Vision Transformers lies in their adeptness at capturing global relationships within an image through self-attention, tailoring the feature extraction process to the specificities of the input data. Unlike ViTs, CNNs \cite{he2016deepresnet, simonyan2014veryvgg16, gao2019res2net} rely on convolutions, which have a local receptive field and are input-agnostic in nature. Although convolutions bring various inductive biases into the network, they cannot identify input-specific characteristics, potentially leading to suboptimal feature extraction for diverse data distributions. Also, these convolutional models have a hierarchical approach to extracting global features, which involves significant downsampling of the input through pooling layers or strides in convolutional layers. Although this downsampling is crucial for achieving a broader receptive field, it significantly loses fine-grained details, which can be critical for tasks requiring high-resolution understanding. Additionally, the hierarchical structure of CNNs struggles to capture long-range dependencies within the input image, as each convolutional layer only processes information from a limited receptive field. Although deeper networks can theoretically capture broader relationships, the loss of detail due to downsampling makes this approach inefficient. Multiple works try to address the above-discussed problems, they are computationally expensive or still follow the same architecture. For example, deformable convolutions \cite{dai2017deformable} try to increase the receptive field of a convolutional kernel such that the weights act on the most critical locations in a feature map. However, they use a convolution layer to sample these locations, and the overall process is computationally expensive. Another work \cite{ding2022scaling} increases the receptive field of individual convolutional weights at each layer but still uses the exact four times downsampling scheme used by other CNN architectures, which is a loss of essential information without significant feature extraction.

% On the other hand, famous CNN architectures \cite{he2016deepresnet, simonyan2014veryvgg16, gao2019res2net} rely on convolutions that are input-agnostic. The weights of convolutional filters in CNNs are learned during the training phase and remain fixed during inference. This static nature means that the same filters are applied regardless of the input's specific characteristics, potentially leading to suboptimal feature extraction for diverse data distributions. Also, these convolutional models have a hierarchical approach to extracting global features, which involves significant downsampling of the input through pooling layers or strides in convolutional layers. Although this downsampling is crucial for achieving a broader receptive field, it significantly loses fine-grained details, which can be critical for tasks requiring high-resolution understanding. Additionally, the hierarchical structure of CNNs struggles to capture long-range dependencies within the input image, as each convolutional layer only processes information from a limited receptive field. Although deeper networks can theoretically capture broader relationships, the loss of detail due to downsampling makes this approach inefficient. Although multiple works try to address the above-discussed problems, they are computationally expensive or still follow the same architecture. For example, deformable convolutions \cite{dai2017deformable} try to increase the receptive field of a convolutional kernel such that the weights act on the most critical locations in a feature map. However, they use a convolution layer to sample these locations, and the overall process is computationally expensive. Another work \cite{ding2022scaling} increases the receptive field of individual convolutional weights at each layer but still uses the exact four times downsampling scheme used by other CNN architectures, which is a loss of essential information without significant feature extraction.

% Pre-trained on the modified COCO dataset, we propose a family of models named \textbf{WideUNet}, a modification of SODAWideNet \cite{dulam2023sodawidenet}. A dense prediction task like SOD requires a model to identify semantically significant features from smaller and larger receptive fields. Hence, we design our models to have two parallel branches that simultaneously extract local and global features. To extract global features, we propose Attention guided Long Range Feature Extraction (AGLRFE), combining dilated convolutions and self-attention to extract long-range features from large spatial resolution feature maps. Unlike MRFFAM in SODAWideNet, we use attention to guide features from dilated convolutions, forcing the convolutional weights to look for semantically rich features. It also instills input dependency into the network, thus bringing in some advantages vision transformers enjoy. On the other hand, convolutions bring in translation equivariance and, therefore, let the proposed models achieve good performance with lesser pre-training data. We utilize the Local Processing Module (CFM) proposed in the SODAWideNet architecture to extract local features. Below, we summarize our contributions.

Pre-trained on the modified COCO dataset, we propose \textbf{SODAWideNet}++, a modified SODAWideNet \cite{dulam2023sodawidenet} architecture that seamlessly integrates Attention into convolutional components. We follow a similar architectural design to SODAWideNet, which separates local and global feature extraction. To extract global features, we combine dilated convolutions from the Multi-Receptive Field Feature Aggregation Module (MRFFAM) and Attention from Multi-scale Attention (MSA) modules and propose Attention guided Long Range Feature Extraction (AGLRFE). Furthermore, we modified the Local Processing Module (LPM) by adding Attention and thus proposed an Attention-enhanced Local Processing Module (ALPM) to extract local features. ALPM comprises smaller $3 \times 3$ convolutional kernels essential for acquiring local features. We reuse the Cross Feature Module (CFM) to combine features from both the proposed components. We summarize our contributions below - 

\begin{enumerate}
    \item We propose SODAWideNet++, a convolutional model utilizing self-attention to extract global features from the beginning of the network.
    \item We modify the famous COCO semantic segmentation dataset to generate binary labels and use it to pre-train the proposed model.
    \item We propose AGLRFE to extract features from large receptive fields using dilated convolutions and Self-Attention.
    \item Unlike prior works, we supervise foreground and background predictions for increased accuracy.
\end{enumerate}

% \textbf{Pre-training in Computer Vision} The idea of pre-training a computer vision network is to learn a universal feature representation that benefits downstream tasks like Semantic Segmentation, Object Detection, etc. Currently, ImageNet \cite{deng2009imagenet} pre-training is the most famous pre-training mechanism for state-of-the-art models in SOD. A backbone network is first pre-trained on the ImageNet dataset, followed by designing task-specific modules to convert backbone features to produce saliency maps. Finally, fine-tuning of both components happens using a SOD dataset like DUTS \cite{wang2017DUTS-TE}. This formulation does not allow pre-training of the backbone and the task-specific elements, which is undesirable. Hence, we concentrate on finding a better pre-training scheme for SOD. To that end, we modify the COCO semantic segmentation dataset \cite{lin2014microsoftcoco} to a SOD dataset by converting multi-class annotations to binary ones. Intuitively, Semantic Segmentation and SOD are very similar. Semantic Segmentation indicates the extent of individual objects in an image and their class information. In contrast, SOD only requires the area of an object in an image. Hence, we utilize the modified COCO dataset to pre-train the proposed models end-to-end and illustrate that this approach is more effective than ImageNet pre-training. Additionally, hyperparameter exploration becomes easier since the nature of pre-training (mod. COCO) is similar to the fine-tuning task (SOD). Figure~\ref{fig:imagenetvscoco} illustrates the fundamental difference between the two approaches.
% Pre-training a neural network with large amounts of data imparts universal feature representation that benefits downstream tasks like Semantic Segmentation, Object Detection, etc. Currently, the most popular method for state-of-the-art models in SOD is ImageNet pre-training \cite{deng2009imagenet}. The process involves pre-training a backbone network on the ImageNet dataset and creating task-specific modules to generate saliency maps from the backbone features. Finally, both components are fine-tuned using a SOD dataset like DUTS \cite{wang2017DUTS-TE}. However, this approach does not allow for pre-training of both the backbone and task-specific elements, which is not ideal. Therefore, we focus on finding a better pre-training scheme for SOD. Since Semantic Segmentation and SOD are similar, with the former being a per-pixel multi-class classification and the latter being a per-pixel binary classification problem, we modify the COCO semantic segmentation dataset \cite{lin2014microsoftcoco} by binarizing annotations to pre-train our model, as shown in Figure \ref{fig:COCO}. This pre-training dataset is quite similar to the fine-tuning dataset, making finding optimal hyperparameters easier. Figure~\ref{fig:imagenetvscoco} illustrates the fundamental difference between the two approaches.

==> chapters/method.tex <==
\section{Proposed Method}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/Architecture.pdf}
    \caption{The proposed architecture \textbf{SODAWideNet++} contains two branches, one to extract global features using AGLRFE and the other to extract local features using ALPM. These global and local features pass through CFM, producing the output of an encoding layer. The decoding layers also consist of two parallel paths, MRFFAM and Identity operation to decode features through multiple receptive fields. The output of every decoder layer is first upsampled by a factor of two, followed by a concatenation of encoder features, and finally refined by a series of convolutions.}
    \label{fig:architecture}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.65\linewidth, height=7.5cm]{images/AGLRFEFinal.pdf}
    \caption{Attention-guided Long-Range Feature Extraction module (AGLRFE) consists of two branches: a collection of dilated convolutions with different dilation rates to extract long-range convolution features and a self-attention block. We reduce the spatial resolution of the input before the Self-Attention block using Average Pooling and refine them using a series of convolution operations. Attention features are then upsampled to the exact resolution as the convolution features from the dilated convolutions. Then, using a series of convolution layers, we bring its channel size to one and pass it through a Sigmoid layer. These features refine our long-range convolution features, thus inducing input-reliance.}
    \label{fig:aglrfe}
\end{figure*}

% The proposed model is a modification of \cite{dulam2023sodawidenet}. We follow their design ideology of extracting global features from large feature maps with minimal corruption of features. This section starts with a brief introduction to SODAWideNet, followed by an introduction to the proposed model SODAWideNet++. Next, we delve into the building blocks of SODAWideNet++, namely AGLRFE and ALPM. Finally, we explain our model's loss function and other intangible aspects. 
The proposed model is an improved version of the design principles introduced in \cite{dulam2023sodawidenet}. This model aims to extract global features from large feature maps with minimal loss of information. In this section, we'll first explain the SODAWideNet model, which serves as the basis for our enhanced model, SODAWideNet++. Then, we'll dive into the core components of SODAWideNet++, namely the Attention Guided Long Range Feature Extraction (AGLRFE) and the Attention Local Pooling Module (ALPM). Finally, we'll discuss the specific loss function used in our model and other essential elements of our design strategy.
% The proposed model is very similar to SODAWideNet \cite{dulam2023sodawidenet}. SODAWideNet is an encoder-decoder-style architecture that extracts long-range features from higher resolutions using dilated convolutions and self-attention. The encoder has three parallel paths, namely the MRFFAM, the MSA, and the LPM, to extract global and local features simultaneously. MRFFAM consists of various dilated convolutions to extract long-range convolutional features, whereas MSA consists of computing self-attention across multiple scales. Having two separate branches to extract global features is parameter-inefficient. Hence, we made significant changes to the model. Firstly, we remove the Multi-Scale Attention modules from the Encoder part of SODAWideNet. Although multi-scale attention is valuable, it is computationally very expensive to compute attention multiple times. Secondly, we modify the MRFFAM module and call it AGLRFE. The later sections will explain More information about the modification from MRFFAM to AGLRFE. These changes reduce the total parameters by 33\%, allowing us to scale the current models. We reused LPM, and CFM proposed in SODAWideNet and followed a similar structure. Thus, the proposed model consists of the neck, the encoder, and the decoder. The neck extracts high-level features and simultaneously reduces the spatial resolution by a factor of two. Subsequently, the two encoder blocks extract local and global features using MRFFAM and LPM, combined by CFM. Each encoder block reduces the spatial resolution by a factor of two, leading to an output stride of eight. Similarly, the decoder blocks refine the encoded features using multiple receptive fields and upsample the feature maps by a factor of two. A concatenation operation before upsampling helps add high-level features to the decoder. All MRFFAM, LPM, and CFM outputs are supervised with ground truth to produce accurate saliency predictions.

\subsection{SODAWideNet}
SODAWideNet, as described in \cite{dulam2023sodawidenet}, employs an encoder-decoder architecture designed to extract long-range features from high-resolution inputs, utilizing dilated convolutions and self-attention mechanisms. The encoder is composed of three parallel pathways: the Multi-Receptive Field Feature Aggregation Module (MRFFAM), the Multi-Scale Attention (MSA), and the Local Processing Module (LPM). These pathways are engineered to capture both global and local features concurrently. In the decoding phase, the architecture features two parallel paths, MRFFAM and Identity, which work together to decode the encoded features and generate the final saliency outputs. The overall architecture consists of two such encoder and decoder blocks. 

\subsection{SODAWideNet++}
SODAWideNet++ builds upon the foundational architecture of SODAWideNet, maintaining distinct branches for extracting local and global features. While SODAWideNet has demonstrated commendable performance when trained from scratch, it still lags behind Sota models in terms of overall efficacy. In SODAWideNet++, we refine the approach of capturing long-range features by merging the functionalities of dilated convolutions and attention into a single, streamlined module named Attention-Guided Long Range Feature Extraction (AGLRFE). This module is engineered to generate long-range, input-dependent convolutional features, thereby enhancing the robustness of the feature representation. Additionally, we incorporate attention into the Local Processing Module (LPM) to increase input dependency, rebranding it as the Attention-enhanced LPM (ALPM). The Combining Feature Module (CFM) remains unchanged and is tasked with the integration and refinement of both local and global features. The decoder structures in SODAWideNet++ and SODAWideNet are identical, preserving the architectural consistency across both models.

\subsection{Attention guided Long Range Feature Extraction (AGLRFE)}
Vision transformers have achieved significant success due to the effectiveness of Self-Attention in extracting important semantic features across large receptive fields. On the other hand, conventional CNNs achieve a global receptive field by downsampling the input hierarchically, which can lead to the loss of critical features and increase the model's parameters. To overcome these limitations, we have employed dilated convolutions with substantial dilation rates to expand the receptive field of our network without increasing the parameter count. However, Self-Attention provides a unique advantage by being intrinsically input-dependent. Thus, to leverage the strengths of both approaches, we propose a hybrid module that combines convolutions and self-attention. We use dilated convolutions to capture extended convolutional features and Self-Attention to derive input-specific features and use them to guide the convolution features. Below, we illustrate particular components of AGLRFE.

\begin{gather*}
    B_{i}(x) = convB_{i}(convB_{i}(x)) \\
    G_{i}(x) = conv_{i}(conv_{i}(x)) \\
    feat = B_{1}(X) \\
    f_{i} = G_{i}(feat) \\
    f_{attention} = Attn(B_{1}(AvgPool(feat)))
\end{gather*}

$convB_{i}$ implies a $3 \times 3$ convolution with dilation $i$ followed by Batch Normalization and GELU activation function, whereas $conv_{i}$ implies a $3 \times 3$ convolution with dilation $i$ followed by Group Normalization and GELU activation function. $AvgPool$ is average pooling with a specific stride of two or four. Before computing the attention features, we apply Average Pooling to reduce the spatial resolution of the input feature map, optimizing the processing efficiency of our model.

\begin{equation*}
    Attn = softmax \left( \frac{K \times Q}{\sqrt{d_{k}}} \right) V
\end{equation*}

where $K, Q$ and $V$ are computed using $conv_{1}(feat)$. Finally, we send the attention features through a couple of convolution layers followed by a sigmoid layer and multiply with feature maps from each dilated convolution. This way, attention values help refine the outputs of each dilated convolution, thus introducing some levels of input dependency in a convolutional neural network.
\begin{equation*}
    f_{conv} =  \{f_{i} + (f_{i} \times \sigma(B_{1}(\uparrow f_{attention})))\} \quad
     \text{where} \quad i \in \{6, 10, 14, 18, 22\}
\end{equation*}

where, $\{\}$ implies a concatenation operation, $\sigma$ is the sigmoid operation, and $i$ belongs to the set of dilation rates. Finally, the output of an AGLRFE is obtained by concatenating the newly generated convolution features and $feat$ and passing these features through a U-net style downsampling operation.

\begin{equation*}
    f_{lr} = B_{1}(MaxPool(\{f_{conv}, feat\}))
\end{equation*}
Figure \ref{fig:aglrfe} shows the architecture of the proposed module.

\subsection{Attention-enhanced Local Processing Module (ALPM)}
The Local Processing Module (LPM) in \cite{dulam2023sodawidenet} employs $3 \times 3$ convolutions to extract local features crucial for precise saliency predictions. This module uses a series of max-pooling layers to identify discriminative features from small neighborhoods, enhancing the model's ability to focus on relevant details. To augment this structure with an added layer of input-specific adaptability, we have refined the LPM by incorporating a Self-Attention mechanism. This Self-Attention is strategically applied to the feature map with the smallest spatial resolution within the LPM, enabling the module to obtain input characteristics from the most informative feature map. 

\begin{gather*}
    fx = MAXPOOL(X) \\
    feat = B_{1}(MAXPOOL(fx)) \\
    fy = B_{1}(\{\uparrow (feat + \textbf{Attn}(feat)), fx\}) \\
    f_{sr} = B_{1}(fx) + fy
\end{gather*}
Above, we illustrate the series of operations in LPM along with the modification highlighted in \textbf{bold}.

\subsection{Model Supervision}
The proposed model generates both contour and saliency predictions at each decoding stage, which are then compared against the ground-truth contour and saliency maps to ensure accuracy. During the encoding stage, outputs from the Attention Guided Long Range Feature Extraction (AGLRFE), the Attention-enhanced Local Processing Module (ALPM), and the Cross Feature Merging (CFM) are also supervised with ground-truth saliency maps for precise predictions. For background supervision, our approach involves an inversion technique where the model outputs are multiplied by -1. This step is crucial as the outputs are subsequently processed through a sigmoid activation layer. The sigmoid function converts these values such that higher values are assigned to pixels belonging to background pixels and lower values to pixels of a salient object. 

\begin{gather*}
    O_{contour}, O_{salient} = SODAWideNet++(X) \\
    O_{bg} = O_{salient} \times -1
\end{gather*}

% \subsection{Variants of the proposed model}
% We use a hyperparameter to control the number of parameters of our model, and to that end, we propose three variants of the proposed WideUNet. \textbf{WideUNet-S} is the smallest model with 1.6M parameters, \textbf{WideUNet-M} is the medium-sized model with 6.4M parameters, and \textbf{WideUNet-L} is the largest variant of the proposed model with 23.4M parameters. All the models use the same set of dilation rates and have the same output stride. The only difference among them is the channel sizes.

\subsection{Loss Function}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/Img.png}
%     \caption{}
%     \label{fig:subim1}
%     \end{subfigure}
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/GT.png}
%     \caption{}
%     \label{fig:subim2}
%     \end{subfigure}
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/BackgroundGT.png}
%     \caption{}
%     \label{fig:subim3}
%     \end{subfigure}
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/AlphaForeground.png}
%     \caption{}
%     \label{fig:subim4}
%     \end{subfigure}
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/SuperimposedAlphaFg.png}
%     \caption{}
%     \label{fig:subim5}
%     \end{subfigure}
%     \begin{subfigure}{0.23\linewidth}
%     \includegraphics[width=1.0\linewidth]{images/SuperimposedAlphaBg.png}
%     \caption{}
%     \label{fig:subim6}
%     \end{subfigure}
    
%     % \includegraphics[width=0.3\linewidth]{images/GT.png}
%     % \includegraphics[width=0.3\linewidth]{images/BackgroundGT.png}
%     % \includegraphics[width=0.3\linewidth]{images/AlphaForeground.png}
%     % \includegraphics[width=0.3\linewidth]{images/SuperimposedAlphaFg.png}
%     % \includegraphics[width=0.3\linewidth]{images/SuperimposedAlphaBg.png}
%     \caption{In this figure, we visualize the alpha values for foreground and background supervision. a) is the input image, b) is the ground-truth saliency map, and c) is the ground-truth background mask. d) indicates the $\alpha^{fg}$ values, e) is the $\alpha^{fg}$ value superimposed over the input, and f) is the $\alpha^{bg}$ value superimposed over the input. Blue in e) and f) indicates higher weights to pixel values, whereas red indicates lower values.}
%     \label{fig:alphavis}
% \end{figure}
% \vspace{-3em}


To train the proposed model, we create a custom loss that directs the model to produce accurate saliency predictions. Following \cite{dulam2023sodawidenet}, our model has saliency and contour outputs, supervised with the ground-truth saliency and contour maps, as shown in Equations \ref{TotalSalLoss} and \ref{TotalConLoss}, respectively.

\begin{equation}\label{TotalSalLoss}
\begin{split}
    L_{salient} = \sum_{i=1}^{2} (L_{AGLRFE_{(i)}}^{sal} + L_{ALPM_{(i)}}^{sal} + L_{CFM_{(i)}}^{sal} \\ + L_{MRFFAM_{(i)}}^{sal} + L_{CFMD_{(i)}}^{sal})
\end{split}
\end{equation}

% \begin{equation}\label{TotalConLoss}
% \begin{split}
%     L_{contour} = \sum_{i=1}^{2} L_{DEC_{(i)}}^{con} \\
%     L^{con} = 0.001 \cdot L_{BCE} + L_{dice} + L_{SSIM}
% \end{split}
% \end{equation}

\begin{equation}\label{TotalConLoss}
\begin{split}
    L_{contour} = L_{MRFFAM_{(1)}}^{con} + L_{MRFFAM_{(2)}}^{con} \\ + L_{CFMD_{(1)}}^{con} + L_{CFMD_{(2)}}^{con} \\
    L^{con} = 0.001 \cdot L_{BCE} + L_{dice} \quad \quad \quad
\end{split}
\end{equation}

where $L_{BCE}$ and $L_{dice}$ are the Binary Cross Entropy and Dice loss, respectively. Unlike other methods, we supervise foreground and background saliency maps. Hence, $L^{sal}$ is divided into two parts. The foreground loss denoted by $L_{fg}$ is the same as the loss function in SODAWideNet, whereas $L_{bg}$ is the newly added background supervision. For COCO pre-training, we set $\beta$ to one, and for DUTS, we set it to 0.5.

\begin{equation}\label{fgbgloss}
    \begin{split}
    L^{sal} = L_{fg} + \beta \cdot L_{bg} \quad \quad \quad \quad \\
        L_{fg} = \alpha^{fg} \cdot L_{bce} + \alpha^{fg} \cdot L_{iou} + \alpha^{fg} \cdot L_{1} \\
        L_{bg} = \alpha^{bg} \cdot L_{bce} + \alpha^{bg} \cdot L_{iou} + \alpha^{bg} \cdot L_{1}
    \end{split}
\end{equation}

where $L_{bce}$, $L_{iou}$, and $L_{1}$ are per-pixel Binary Cross Entropy, Intersection-over-Union, and L1 losses, respectively. $\alpha_{ij}^{fg}$ and $\alpha_{ij}^{bg}$ are per-pixel weights determined for each pixel during foreground and background supervision. Per-pixel weights ensure that wrong predictions for specific pixels are penalized heavily. Below, we illustrate the procedure to compute these values. Both $\alpha^{fg}$ and $\alpha^{bg}$ have the exact spatial resolution as the output. Hence, we compute pixel-wise loss in Equation \ref{fgbgloss} and multiply them with $\alpha$. 
\begin{gather*}
    \alpha_{ij}^{fg} = max(GT_{ij})_{31 \times 31} \\
    \alpha_{ij}^{bg} = BackgroundGT_{ij} \\
    BackgroundGT = \mathds{1}\ - GT
\end{gather*}
$\alpha_{ij}^{fg}$ for a pixel at spatial location $(i, j)$ is calculated by finding the largest value in a $31 \times 31$ window centered on that pixel location. Whereas $\alpha_{ij}^{bg}$ equals the pixel's intensity value in the background map. Figure \ref{fig:AlphaBetaImage} indicates the values of $\alpha_{ij}^{fg}$ and $\alpha_{ij}^{bg}$ superimposed on the input. Finally, from Equations \ref{TotalSalLoss}, and \ref{TotalConLoss}, the total loss to train our model is given as

\begin{equation} \label{TotalLoss}
    L_{total} = L_{salient} + L_{contour} %+ L_{siamese}
\end{equation}

\begin{figure*}[ht!]
    \centering
    \begin{tikzpicture}[
 image/.style = {text width=0.165\linewidth,
                 inner sep=0pt, outer sep=0pt},
node distance = 0mm and 0mm
                        ]

\node [image] (frame11)
    {\includegraphics[width=\linewidth]{images/Img.png}};
\node [image, right=of frame11] (frame21) 
    {\includegraphics[width=\linewidth]{images/GT.png}};
\node [image, right=of frame21] (frame31) 
    {\includegraphics[width=\linewidth]{images/BackgroundGT.png}};
\node [image, right=of frame31] (frame41) 
    {\includegraphics[width=\linewidth]{images/AlphaForeground.png}};
\node [image, right=of frame41] (frame51) 
    {\includegraphics[width=\linewidth]{images/SuperimposedAlphaFg.png}};
\node [image, right=of frame51] (frame61) 
    {\includegraphics[width=\linewidth]{images/SuperimposedAlphaBg.png}};

\node[below=of frame11]{\tiny I};
\node[below=of frame21]{\tiny FG};
\node[below=of frame31]{\tiny BG($\alpha_{ij}^{bg}$)};
\node[below=of frame41]{\tiny $\alpha_{ij}^{fg}$};
\node[below=of frame51]{\tiny $\alpha_{ij}^{fg}$ SI};
\node[below=of frame61]{\tiny $\alpha_{ij}^{bg}$ SI};


\end{tikzpicture}
    \caption{In the above figure, we visually illustrate the pixels that receive a higher weight for loss computation as shown in equation \ref{fgbgloss}. The image illustrates in white the pixels that receive a higher weight for the background loss, and the fourth image illustrates the pixels receiving a higher weight to compute the foreground loss. The last two images depict the important pixels (in blue) superimposed (SI) on the input image.}
    \label{fig:AlphaBetaImage}
\end{figure*}

==> chapters/related_works.tex <==
\section{Related Works}

\subsection{Salient Object Detection with ImageNet pre-training}

PiCANet-R~\cite{liu2018picanet} developed a contextual attention module to attend to essential context locations for every pixel from Resnet-50 features. BASNet \cite{qin2019basnet} uses an encoder-decoder-style network initialized by a Resnet-34 model and a boundary refinement network on top to produce accurate saliency predictions with crisp boundaries. F3-Net \cite{wei2020f3net} uses a Resnet-50 network to extract semantic features refined by a cascaded feedback decoder (CFD) and cross-feature module to produce saliency outputs. VST \cite{Liu_2021_ICCV_VST} is the first work to propose a vision transformer-based SOD model. PSG uses a loss function that creates auxiliary saliency maps based on the morphological closing operation to generate accurate saliency maps incrementally. EnergyTransf \cite{jing_ebm_sod21generative} uses an energy-based prior for salient object detection. RCSB \cite{Ke_2022_WACV_RCSB} refines features extracted from a Resnet-50 \cite{he2016deepresnet} backbone using Stage-wise Feature Extraction (SFE) and a few novel loss functions for SOD. CS-Net \cite{gao2020sod100kcsf} proposes a flexible convolutional module named gOctConv to utilize multi-scale features for SOD. EDNet \cite{wu2022edn} presents a novel downsampling technique to learn a global view of the whole image to generate high-level features for SOD. PGNet uses a combination of Resnet and Swin\cite{liu2021swin} models to generate saliency maps. ICON \cite{zhuge2021salienticon} introduces a diverse feature aggregation (DFA) component to aggregate features with various receptive fields and increase the feature diversity. TRACER \cite{lee2022tracer} uses an EfficientNet backbone and attention-guided tracing modules to detect salient objects. LDF \cite{ldf} proposes a label decoupling framework to detect salient objects. The authors disintegrate the original saliency map into body and detail maps to concentrate on the central object and object edges separately. PA-KRN \cite{pakrn} uses a knowledge review network to first identify the salient object and then segment it. RMFormer \cite{rmformer} proposes a novel Recurrent Multi-scale transformer that utilizes a transformer and multi-scale refinement architectures for SOD. 


% \subsection{Pre-training for Downstream Vision tasks}

% ImageNet pre-training has been the de facto mechanism to equip computer vision models with the knowledge beneficial to achieve good performance on downstream tasks like Semantic Segmentation, Object Detection, SOD, etc. ImageNet pre-training is a two-step procedure where the first step involves training an image classification network called the backbone. In the second step, task-specific modules are added to the backbone and fine-tuned on a target task. Fine-tuning on a downstream task like Semantic Segmentation does not allow the backbone and task-specific components to be pre-trained on ImageNet. Masked Auto-Encoding (MAE) \cite{woo2023convnextv2} is a more recent form of pre-training where a network takes in a masked version of an image and outputs a reconstructed image. Although this paradigm allows combining the backbone and task-specific components, it still requires vast data. Different from these techniques, we utilize a supervised pre-training scheme in our work. We modify the famous COCO Semantic Segmentation dataset and turn it into a SOD dataset. Specifically, we binarize the annotations of each image, thus turning it into a 118k images extensive supervised SOD dataset. 

\subsection{Combining Convolutions and Attention}

Combining convolutions and attention, two fundamental concepts in computer vision, is an exciting research direction. Xiao \textit{et al}.~\cite{xiao2021early} was one of the first works to use a convolutional stem before a transformer architecture for adding inductive biases. Wu \textit{et al}.~\cite{wu2021cvt} replaced positional embedding in vision transformers using convolutions to generate the key, query, and value matrices. Many works~\cite{xie2021segformer,liu2021swin} have since followed suit. Pan \textit{et al}.~\cite{pan2022integrationacmix} (ACmix) proposes a hybrid module containing convolutions and attention in parallel. Bello \textit{et al}.~\cite{bello2019attentionaugmented} proposed Attention-augmented convolutions, which introduce a novel two-dimensional relative self-attention mechanism that replaces convolutions as a computational primitive. Gulati \textit{et al}.~\cite{gulati2020conformer} (Conformer) modifies the original self-attention block with a novel convolutional block consisting of depthwise convolutions. Yuan \textit{et al}.~\cite{yuan2021incorporatingceit} proposed a Convolution-enhanced image Transformer (CeiT) that uses convolutions to extract patch features using Image-2-tokens and modify the feed-forward network in the transformer block. Dulam \textit{et al}.~\cite{dulam2023convsegformer} modifies the SegFormer~\cite{xie2021segformer} architecture by adding a convolutional stem and a U-Net-style convolutional decoder. 

==> chapters/revision_text.tex <==
\section{Revision}
\label{sec:revision}

We thank all the reviewers for their constructive comments: We thank R1 \& R3 for finding our work novel with sufficient experimental evaluation. As per R1, we have removed the associated section. We thank R2 for identifying two of our contributions and suggesting more experiments. We accommodated all of these valuable comments in the revised paper.

% In response to the reviewers' queries, we provide additional experiments to further highlight the significance of SODAWideNet++.

\subsection{Reviewer 2 Comments}

\textbf{\textit{Comparison with state-of-the-art methods in 2023}}

We thank the reviewer for their suggestion to include the $E$-measure and the weighted F-measures in the main table, along with a comparison to SOD models in 2023.
In Tables \ref{tab:ResultsTable20231} and \ref{tab:ResultsTable20232}, we have added performance numbers of SODAWideNet++ (Ours) against state-of-the-art methods in 2023 (SelfReformer (SR) \cite{SelfReformer} and RMFormer (RM) \cite{rmformer}). Further, we have added results from the most recent method from CVPR 2024 (VSCode (VSC) \cite{luo2024vscode}). 

% Although other models outperform SODAWideNet++ on several metrics, SODAWideNet++ stands out for its efficiency, using significantly fewer parameters coupled with a significantly smaller pre-training pipeline while still delivering competitive results. For example, SODAWideNet++ contains only 33\% of trainable parameters compared to the state-of-the-art RMFormer, 35\% of trainable parameters compared to VSCode, and only 12\% of trainable parameters compared to SelfReformer-SWIN. These rows will be added to the main comparison table.

SODAWideNet++ uses significantly fewer parameters and a smaller pre-training pipeline, delivering competitive results. For example, SODAWideNet++ contains only \textbf{33\%}, \textbf{35\%}, and \textbf{13\%} of trainable parameters compared to the state-of-the-art RMFormer, VSCode, and SelfReformer, respectively. These rows will be added to the main table.

\vspace{-4mm}

 \begin{table*}[ht!]
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{|c|c|cccc|cccc|cccc|}
    \hline
      Method& Params. (M)&  \multicolumn{4}{c|}{DUTS-TE} & \multicolumn{4}{c|}{DUT-OMRON} & \multicolumn{4}{c|}{HKU-IS} \\
    \hline
     & & $F_{max}$ & MAE  & $S_{m}$ & $E_{m}$ & $F_{max}$ & MAE & $S_{m}$ & $E_{m}$ &
    $F_{max}$ & MAE &  $S_{m}$ & $E_{m}$ \\
    \hline

    SRr$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.925& 0.024&0.921 & 0.924&
    0.838&0.043&0.859 & 0.884&
    0.951&0.023&0.934&0.962 \\
    
    RM$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&
    0.931& 0.023&0.925 & 0.933&
    0.861&0.040&0.877 & 0.904&
    0.957&0.019&0.940&0.968 \\

    VSC$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.931& 0.024&0.926 & 0.931&
    0.861&0.042&0.876 & 0.899&
    0.957&0.021&0.940&0.965 \\

    \hline

    \textbf{Ours} & \textbf{26.58}&
    \textbf{0.917}& \textbf{0.029}&\textbf{0.910} &\textbf{0.916} & 
    \textbf{0.848}&\textbf{0.045}&\textbf{0.868} &\textbf{0.896} & 
    \textbf{0.950}&\textbf{0.024}&\textbf{0.932}
    &\textbf{0.960} \\
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on DUTS-TE, DUT-OMRON, and HKU-IS datasets.}
  \label{tab:ResultsTable20231}
\end{table*}
\vspace{-12mm}

\begin{table*}[ht!]
  \centering
  \begin{adjustbox}{width=0.8\linewidth}
  \begin{tabular}{|c|c|cccc|cccc|}
    \hline
      Method& Params. (M) & \multicolumn{4}{c|}{ECSSD} & \multicolumn{4}{c|}{PASCAL-S}\\
    \hline
     & &
    $F_{max}$ & MAE &  $S_{m}$  & $E_{m}$  &
    $F_{max}$ & MAE &  $S_{m}$ &  $E_{m}$ \\
    \hline

    SR$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.962&0.025&0.941 & 0.935&
    -&-&-&-\\
    
    RM$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&
    0.964&0.020&0.947 & 0.938&
    -&-&-&-\\

    VSC$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.965&0.021&0.949 & 0.934&
    0.912&0.051&0.885&0.870\\

    \hline

    \textbf{Ours} & \textbf{26.58}&
   \textbf{ 0.957}&\textbf{0.029}&\textbf{0.935} &\textbf{0.927} & 
    \textbf{0.901}&\textbf{0.062}&\textbf{0.875}&\textbf{0.870}\\

    
    % \midrule
    % \bottomrule
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on ECSSD and PASCAL-S datasets.}
  \label{tab:ResultsTable20232}
\end{table*}
\vspace{-8mm}

\noindent\textbf{\textit{Pre-training another model using the modified COCO dataset}}

We pre-train the PGN \cite{xie2022pyramid} method using the modified COCO dataset without their ImageNet pre-trained weights. Tables \ref{tab:pgnet1} and \ref{tab:pgnet2} contain a quantitative evaluation of the COCO pre-trained PGN, ImageNet pre-trained PGN, and PGN trained from scratch on the DUTS dataset. We have included our model for comparison. Pre-training using the COCO dataset significantly outperforms training from scratch and delivers competitive results against the ImageNet pre-trained PGN model. 

\begin{table*}[ht!]
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{|c|c|ccccc|ccccc|ccccc|}
    \hline
      Method& Params. (M)&  \multicolumn{5}{c|}{DUTS-TE} & \multicolumn{5}{c|}{DUT-OMRON} & \multicolumn{5}{c|}{HKU-IS} \\
    \hline
     & & $F_{max}$ & MAE  & $S_{m}$ & $E_{m}$ & $E_{m}$ & $F_{max}$ & MAE & $S_{m}$ & $E_{m}$ & $E_{m}$ &
    $F_{max}$ & MAE &  $S_{m}$ & $E_{m}$ &$E_{m}$  \\
    \hline

    PGN$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.917& 0.027&0.911 & 0.922&0.874&
    0.835&0.045&0.855 & 0.887&0.775&
    0.948&0.024&0.929&0.961&0.916 \\

    PGN-COCO$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.882& 0.040&0.879 & 0.896& 0.820&
    0.803&0.057&0.828 & 0.859&0.732&
    0.931&0.031&0.912&0.948&0.732 \\

    \hline

    \textbf{Ours} & \textbf{26.58}&
    \textbf{0.917}& \textbf{0.029}&\textbf{0.910} &\textbf{0.916}&\textbf{0.916} & 
    \textbf{0.848}&\textbf{0.045}&\textbf{0.868} &\textbf{0.896}&\textbf{0.916} & 
    \textbf{0.950}&\textbf{0.024}&\textbf{0.932}
    &\textbf{0.960}&\textbf{0.916} \\
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on DUTS-TE, DUT-OMRON, and HKU-IS datasets.}
  \label{tab:pgnet1}
\end{table*}
\vspace{-12mm}

\begin{table*}[ht!]
  \centering
  \begin{adjustbox}{width=0.8\linewidth}
  \begin{tabular}{|c|c|ccccc|ccccc|}
    \hline
      Method& Params. (M) & \multicolumn{5}{c|}{ECSSD} & \multicolumn{5}{c|}{PASCAL-S}\\
    \hline
     & &
    $F_{max}$ & MAE &  $S_{m}$  & $E_{m}$  & $F_{w}$  &
    $F_{max}$ & MAE &  $S_{m}$ &  $E_{m}$ & $F_{w}$  \\
    \hline

    PGN$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.960&0.027&0.938 & 0.932& 0.929 &
    0.904&0.056&0.874&0.878 &0.849\\

    PGN-COCO$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.940&0.039&0.913 & 0.915& 0.896 &
    0.878&0.069&0.852&0.864&0.818\\

    \hline

    \textbf{SODAWideNet++} & \textbf{26.58}&
   \textbf{ 0.957}&\textbf{0.029}&\textbf{0.935} & 0.927 & 0.922&
   \textbf{0.901}&\textbf{0.062}&\textbf{0.875}&\textbf{0.870} &0.845\\

    
    % \midrule
    % \bottomrule
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on ECSSD and PASCAL-S datasets.}
  \label{tab:pgnet2}
\end{table*}
\vspace{-8mm}
\noindent \textbf{\textit{Ablation experiments corresponding to ALGRFE, ALPM, CFM, \& MRFFAM}}

We express our gratitude to the reviewer for recommending the ablation experiments, which have provided valuable insights into the proposed architecture. Table \ref{tab:components} provides a numerical representation of these insights. The absence of AGLRFE (row one) reduces the model's ability to capture long-range dependencies, leading to the lowest performance across all configurations. The removal of ALPM (row two) reduces the model's ability to capture local features. Similarly, removing CFM (row three) causes a similar decline in performance due to the lack of a complex way to integrate local and global features. Also, removing MRFFAM (row four) on the decoder side results in degraded performance, reinforcing the importance of using various receptive fields to decode features. The inclusion of all the four components produces the best model.
% Table \ref{tab:components} illustrates the effects of the four components of the SODAWideNet++ architecture.
\vspace{-3mm}
\begin{table}[h!]
\centering
  \begin{tabular}{|c|c|c|c|c|c|}%|ccccc}
    \hline
      AGLRFE  & ALPM& CFM & MRFFAM & $F_{max}$ & MAE \\  %\multicolumn{5}{c}{SOD}\\
    \hline
     $\times$& \checkmark & \checkmark & \checkmark& 0.902 & 0.035 \\
    % \hline
    \checkmark  & $\times$ & \checkmark & \checkmark&  0.907 & 0.033 \\
    % \hline
    \checkmark  & \checkmark & $\times$& \checkmark&  0.908 & 0.032\\
    % \hline
    \checkmark  & \checkmark & \checkmark& $\times$&  0.906 & 0.032\\
    % \hline
    \checkmark &  \checkmark & \checkmark& \checkmark& \textbf{0.917} & \textbf{0.029}\\
    \hline
  \end{tabular}
  % \end{adjustbox}
  \caption{Influence of individual components in SODAWideNet++.}
  \label{tab:components}
 \end{table}
\vspace{-9mm}


\noindent \textbf{\textit{Difference from the previous loss pipelines}}

 Prior works only focused on supervising the foreground (saliency) maps, whereas we supervised both the foreground (fg) and background (bg) maps. As seen from Table \ref{tab:bglosssupervision}, background supervision slightly improves performance over foreground supervision.

  \begin{table}[h!]
\centering
  \begin{tabular}{|c|c|c|}%|ccccc}
    \hline
      AGLRFE  & $F_{max}$ & MAE \\  %\multicolumn{5}{c}{SOD}\\
    \hline
     fg + bg & 0.917 & 0.029 \\
     fg & 0.911 & 0.031 \\
    \hline
  \end{tabular}
  % \end{adjustbox}
  \caption{Influence of background (bg) supervision on SODAWideNet++.}
  \label{tab:bglosssupervision}
 \end{table}
\vspace{-5mm}

\subsection{Reviewer 3 Comments}

We thank the reviewer for the exciting research directions, such as Implicit Neural Representation (INR) or the Mamba module for Salient Object Detection.
\\ \\
\textbf{\textit{Highlight how the proposed technique is important and what is key novelty comparing to existing approaches?}}

The proposed SODAWideNet++ is explicitly designed for SOD, unlike prior models that rely on ImageNet pre-trained backbones built primarily for image classification. 
The importance of this tailored design technique is in allowing the simultaneous pre-training of the entire network, encouraging the use of dense prediction based pre-training pipelines for SOD while eliminating the computationally expensive classification-centric ImageNet pre-training.

Our work has three key novel contributions: 1) We combine dilated convolutions and self-attention into a single unit, whereas prior work PGNet \cite{xie2022pyramid} uses separate branches (Swin \cite{liu2021swin} and ResNet \cite{he2016deepresnet}) as feature extractors. 2) To the best of our knowledge, we are the first to use both foreground (saliency) and background maps to generate better saliency predictions. 3) We introduce a dense pre-training pipeline by modifying the COCO semantic segmentation dataset.
% by modifying the COCO semantic segmentation dataset.
\\

% 3) We are the first to modify the COCO semantic segmentation dataset to pre-train SODAWideNet++, replacing the traditional ImageNet classification pre-training.
% Secondly, we supervise both foreground (saliency) and background maps to generate better saliency predictions. Finally, our novel dense pre-training pipeline using the COCO semantic segmentation dataset replacing the traditional

% Finally, we modify the COCO semantic segmentation dataset to pre-train the proposed SODAWideNet++, demonstrating a novel dense pre-training pipeline to replace the traditional ImageNet classification pre-training.

% Unlike traditional models that rely on ImageNet pre-trained backbones, SODAWideNet++ is explicitly designed for SOD, allowing for the pre-training of the entire network simultaneously. This eliminates computationally expensive ImageNet pre-training. Additionally, SOD-specific choices, such as capturing global features with minimal information loss, have resulted in a competitive yet lightweight model compared to other state-of-the-art models.

% Additionally, our model is lightweight compared to other state-of-the-art models, highlighting the advantages of domain-specific architectures, hence the importance of our proposed technique.

% % All the prior works in SOD are built on top of an ImageNet pre-trained backbone built particularly to perform well for Image Classification, a significantly distinct task from SOD. In contrast, we concentrate on creating a network made of components essential for a dense prediction task like SOD. This reduces reliance on ImageNet pre-training, which is very expensive and unfeasible with limited computing power. 

% The proposed Attention Guided Long Range Feature Extraction (AGLRFE) combines large dilated convolutions and self-attention into a single streamlined module that extracts long-range features. This combination leverages convolution operations' inductive biases and self-attention's input dependency to effectively identify salient objects of various sizes. For example, PGNet \cite{xie2022pyramid} uses separate convolution (ResNet) and attention (Swin) networks. Additionally, we supervise both foreground and background predictions. This dual supervision ensures the model generates more precise saliency maps by accurately distinguishing between salient objects and background regions. The influence of adding background supervision can be seen in Table \ref{tab:bglosssupervision}.
% Also, the proposed module, Attention Guided Long Range Feature Extraction (AGLRFE), combines large dilated convolutions and self-attention into a single streamlined module that extracts long-range features. This combination leverages convolution operations' inductive biases and self-attention's input dependency to effectively identify salient objects of various sizes. For example, PGNet \cite{xie2022pyramid} uses separate convolution (ResNet) and attention (Swin) networks. Additionally, we supervise both foreground and background predictions. This dual supervision ensures the model generates more precise saliency maps by accurately distinguishing between salient objects and background regions. The influence of adding background supervision can be seen in Table \ref{tab:bglosssupervision}.
\noindent\textbf{\textit{How is the generalization ability of this work? Especially in scenes with complex backgrounds or with multiple salient objects.}}

% SODAWideNet++'s architecture, combining dilated convolutions and self-attention, is well-suited to handle varied scenes and conditions, enabling it to capture local and global features effectively. This design makes the model robust in detecting salient objects, even in complex backgrounds or when multiple objects are present. Its competitive performance on several datasets, achieving high scores in F-measure (Fmax), Mean Absolute Error (MAE), and S-measure (Sm), further demonstrates its robustness. 

Visual results confirm that SODAWideNet++ can detect salient objects in challenging scenarios, including images with large foreground objects (figure 4 rows one \& four), multiple objects (figure 4 row two), and complex backgrounds (figure 4 row three), showcasing its strong generalization ability. Also, SODAWideNet++'s competitive performance, as shown in Table 1, in terms of F-measure ($F_{max}$), S-measure ($S_{m}$), MAE, and E-measure ($E_{m}$), reiterates its robustness.
\\ \\
\textbf{\textit{Can this model be further extended and applied to 360 VR images or videos? Even in multimodal situations, such as audio-visual saliency detection?}}

Although not designed for 360 VR, we believe our model is adaptable and can be extended to deal with the more complex field of view and spatial relationships of VR data. It would be exciting to extend our method to accommodate extra modalities in multimodal saliency detection tasks.

% We also believe extra modalities such as audio, can enhance the model's performance in multimodal (audio-visual) saliency detection tasks.

% The model's ability to capture long-range dependencies and local features using AGLRFE and ALPM modules makes it adaptable to the unique challenges of 360 VR content, where the field of view and spatial relationships are more complex. Additionally, extra modalities, such as audio, could enhance the model's performance in multimodal saliency detection tasks. The self-attention mechanisms used in SODAWideNet++ can be extended to process and integrate features from multiple modalities, leveraging audio cues to improve visual saliency detection.

% Additionally, all the prior works in SOD are built on top of an ImageNet pre-trained backbone built particularly to perform well for Image Classification, a significantly distinct task from SOD. In contrast, we concentrate on creating a network made of components essential for a dense prediction task like SOD. This reduces reliance on ImageNet pre-training, which is very expensive and unfeasible with limited computing power.

% Also, simultaneously supervising the foreground and background is novel and adds an extra penalty to the model for inaccurate predictions.

% Yes, in future work, we will try to utilize Implicit Neural Representations and Mamba for SOD.

% The proposed SODAWideNet++ performs better on various datasets with complex backgrounds (DUT-OMRON, HKU-IS, and ECSSD) and images with multiple objects (PASCAL-S).

==> revised_chapters/revision_text.tex <==
\section{Revision}
\label{sec:revision}

Firstly, we thank the reviewers for their constructive comments: We thank R1 \& R3 for finding our work novel and state of the art and for sufficient experimental evaluation. In response to the reviewers' queries, we provide additional experiments to further highlight the significance of SODAWideNet++.

\subsection{Reviewer 2 Comments}

\textbf{\textit{Comparison with state-of-the-art methods in 2023}}

We thank the reviewer for their suggestion to include the $E$-measure and the weighted F-measures in the main table, along with a comparison to SOD models in 2023.
In Tables \ref{tab:ResultsTable20231} and \ref{tab:ResultsTable20232}, we have added performance numbers of SODAWideNet++ against state-of-the-art models in 2023 (SelfReformer \cite{SelfReformer} and RMFormer \cite{rmformer}). Further, we have added results from the most recent state-of-the-art model from CVPR 2024 (VSCode \cite{luo2024vscode}). 

% Although other models outperform SODAWideNet++ on several metrics, SODAWideNet++ stands out for its efficiency, using significantly fewer parameters coupled with a significantly smaller pre-training pipeline while still delivering competitive results. For example, SODAWideNet++ contains only 33\% of trainable parameters compared to the state-of-the-art RMFormer, 35\% of trainable parameters compared to VSCode, and only 12\% of trainable parameters compared to SelfReformer-SWIN. These rows will be added to the main comparison table.

SODAWideNet++ uses significantly fewer parameters and a significantly smaller pre-training pipeline, delivering competitive results. For example, SODAWideNet++ contains only \textbf{33\%}, \textbf{35\%}, and \textbf{13\%} of trainable parameters compared to the state-of-the-art RMFormer, VSCode, and SelfReformer, respectively. These rows will be added to the main comparison table.

 \begin{table*}[ht!]
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{|c|c|cccc|cccc|cccc|}
    \hline
      Method& Params. (M)&  \multicolumn{4}{c|}{DUTS-TE~\cite{wang2017DUTS-TE}} & \multicolumn{4}{c|}{DUT-OMRON~\cite{yang2013saliencyOMRON}} & \multicolumn{4}{c|}{HKU-IS~\cite{LiYu15HKU}} \\
    \hline
     & & $F_{max}$ & MAE  & $S_{m}$ & $E_{m}$ & $F_{max}$ & MAE & $S_{m}$ & $E_{m}$ &
    $F_{max}$ & MAE &  $S_{m}$ & $E_{m}$ \\
    \hline

    SelfReformer$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.925& 0.024&0.921 & 0.924&
    0.838&0.043&0.859 & 0.884&
    0.951&0.023&0.934&0.962 \\
    
    RMFormer$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&
    0.931& 0.023&0.925 & 0.933&
    0.861&0.040&0.877 & 0.904&
    0.957&0.019&0.940&0.968 \\

    VSCode$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.931& 0.024&0.926 & 0.931&
    0.861&0.042&0.876 & 0.899&
    0.957&0.021&0.940&0.965 \\

    \hline

    \textbf{SODAWideNet++} & \textbf{26.58}&
    \textbf{0.917}& \textbf{0.029}&\textbf{0.910} &\textbf{0.916} & 
    \textbf{0.848}&\textbf{0.045}&\textbf{0.868} &\textbf{0.896} & 
    \textbf{0.950}&\textbf{0.024}&\textbf{0.932}
    &\textbf{0.960} \\
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on DUTS-TE, DUT-OMRON, and HKU-IS datasets.}
  \label{tab:ResultsTable20231}
\end{table*}
\vspace{-12mm}

\begin{table*}[ht!]
  \centering
  \begin{adjustbox}{width=0.8\linewidth}
  \begin{tabular}{|c|c|cccc|cccc|}
    \hline
      Method& Params. (M) & \multicolumn{4}{c|}{ECSSD~\cite{shi2015hierarchicalECSSD}} & \multicolumn{4}{c|}{PASCAL-S~\cite{li2014secretsPASCAL-S}}\\
    \hline
     & &
    $F_{max}$ & MAE &  $S_{m}$  & $E_{m}$  &
    $F_{max}$ & MAE &  $S_{m}$ &  $E_{m}$ \\
    \hline

    SelfReformer$_{\text{TMM'23}}$~\cite{SelfReformer} & 220&
    0.962&0.025&0.941 & 0.935&
    -&-&-&-\\
    
    RMFormer$_{\text{ACMMM'23}}$~\cite{rmformer} & 87.52&
    0.964&0.020&0.947 & 0.938&
    -&-&-&-\\

    VSCode$_{\text{CVPR'24}}$~\cite{luo2024vscode} & 74.72&
    0.965&0.021&0.949 & 0.934&
    0.912&0.051&0.885&0.870\\

    \hline

    \textbf{SODAWideNet++} & \textbf{26.58}&
   \textbf{ 0.957}&\textbf{0.029}&\textbf{0.935} &\textbf{0.927} & 
    \textbf{0.901}&\textbf{0.062}&\textbf{0.875}&\textbf{0.870}\\

    
    % \midrule
    % \bottomrule
    \hline
  \end{tabular}
  \end{adjustbox}
  % \vspace{-5mm}
  \caption{Comparison of our method with 14 other methods in terms of max F-measure $F_{max}$, MAE, and $S_{m}$ measures on ECSSD and PASCAL-S datasets.}
  \label{tab:ResultsTable20232}
\end{table*}
\vspace{-7mm}


% \begin{table*}[h!]
% \centering
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{|c|c|c|c|c|c|}
%   \hline
%   \textbf{Dataset} & \textbf{Metric} & \textbf{SelfReformer} & \textbf{RMFormer} & \textbf{VSCode} & \textbf{SODAWideNet++} \\
%   \hline
%   \multirow{2}{*}{} 
%   & \textbf{Venue} & TMM'23 & ACMMM'23 & CVPR'24 & - \\
%   \hline
%   \multirow{2}{*}{}
%   & \textbf{Params. (M)} & 220 & 87.52 & 74.72 & \textbf{26.58} \\
%   \hline
%   \multirow{5}{*}{\textbf{DUTS-TE~\cite{wang2017DUTS-TE}}}
%   & $F_{max}$ $\uparrow$ & 0.925 & 0.931 & 0.931 & \textbf{0.917} \\
%   & MAE $\downarrow$ &  0.024 & 0.023 & 0.024 & \textbf{0.029} \\
%   & $S_{m}$ $\uparrow$ & 0.921 & 0.925 & 0.926 & \textbf{0.910} \\
%   & $E_{m}$ $\uparrow$ & 0.924 & 0.933 & 0.931 & \textbf{0.916} \\
%   \hline
%   \multirow{5}{*}{\textbf{DUT-OMRON~\cite{yang2013saliencyOMRON}}}
%   & $F_{max}$ $\uparrow$ & 0.838 & 0.861 & 0.861 & \textbf{0.848} \\
%   & MAE $\downarrow$ & 0.043 & 0.040 & 0.042 & \textbf{0.045} \\
%   & $S_{m}$ $\uparrow$ & 0.859 & 0.877 & 0.876 & \textbf{0.868} \\
%   & $E_{m}$ $\uparrow$ & 0.884 & 0.904 & 0.899 & \textbf{0.896} \\
%   \hline
%   \multirow{5}{*}{\textbf{HKU-IS~\cite{LiYu15HKU}}}
%   & $F_{max}$ $\uparrow$ & 0.951 & 0.957 & 0.957 & \textbf{0.950} \\
%   & MAE $\downarrow$ & 0.023 & 0.019 & 0.021 & \textbf{0.024} \\
%   & $S_{m}$ $\uparrow$ & 0.934 & 0.940 & 0.940 & \textbf{0.932} \\
%   & $E_{m}$ $\uparrow$ & 0.962 & 0.968 & 0.965 & \textbf{0.960} \\
%   \hline
%   \multirow{5}{*}{\textbf{ECSSD~\cite{shi2015hierarchicalECSSD}}}
%   & $F_{max}$ $\uparrow$ & 0.0962 & 0.964 & 0.965 & \textbf{0.957} \\
%   & MAE $\downarrow$ & 0.025 & 0.020 & 0.021 & \textbf{0.029} \\
%   & $S_{m}$ $\uparrow$ & 0.941 & 0.947 & 0.949 & \textbf{0.935} \\
%   & $E_{m}$ $\uparrow$ & 0.935 & 0.938 & 0.934 & \textbf{0.927} \\
%   \hline
%   \multirow{5}{*}{\textbf{PASCAL-S~\cite{li2014secretsPASCAL-S}}}
%   & $F_{max}$ $\uparrow$ & - & - & 0.912 & \textbf{0.901} \\
%   & MAE $\downarrow$ & - & - & 0.051 & \textbf{0.062} \\
%   & $S_{m}$ $\uparrow$ & - & - & 0.885 & \textbf{0.875} \\
%   & $E_{m}$ $\uparrow$ & - & - & 0.870 & \textbf{0.870} \\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison of our method with other methods in terms of max F-measure $F_{max}$, MAE, $S_{m}$, and $E_{m}$ measures on DUTS-TE, DUT-OMRON, HKU-IS, ECSSD, and PASCAL-S datasets.}
% \label{tab:TransposedResultsTable}
% \end{table*}

\noindent \textbf{\textit{Ablation experiments corresponding to ALGRFE, ALPM, CFM, \& MRFFAM}}

We express our gratitude to the reviewers for recommending the ablation experiments, which have provided valuable insights into the proposed architecture. Table \ref{tab:components} provides a numerical representation of these insights. All the results are on the DUTS test split. The absence of AGLRFE (row one) reduces the model's ability to capture long-range dependencies, leading to the lowest performance across all configurations. The removal of ALPM (row two) reduces the model's ability to capture local features. Similarly, removing CFM (row three) causes a similar decline in performance due to the lack of a complex way to integrate local and global features. Also, removing MRFFAM (row four) on the decoder side results in degraded performance, reinforcing the importance of using various receptive fields to decode features. The inclusion of all the four components produces the best model.
% Table \ref{tab:components} illustrates the effects of the four components of the SODAWideNet++ architecture.
\begin{table}[h!]
\centering
  \begin{tabular}{|c|c|c|c|c|c|}%|ccccc}
    \hline
      AGLRFE  & ALPM& CFM & MRFFAM & $F_{max}$ & MAE \\  %\multicolumn{5}{c}{SOD}\\
    \hline
     $\times$& \checkmark & \checkmark & \checkmark& 0.902 & 0.035 \\
    % \hline
    \checkmark  & $\times$ & \checkmark & \checkmark&  0.907 & 0.033 \\
    % \hline
    \checkmark  & \checkmark & $\times$& \checkmark&  0.908 & 0.032\\
    % \hline
    \checkmark  & \checkmark & \checkmark& $\times$&  0.906 & 0.032\\
    % \hline
    \checkmark &  \checkmark & \checkmark& \checkmark& \textbf{0.917} & \textbf{0.029}\\
    \hline
  \end{tabular}
  % \end{adjustbox}
  \caption{Influence of individual components in SODAWideNet++.}
  \label{tab:components}
 \end{table}
\vspace{-7mm}


\noindent \textbf{\textit{Difference from the previous loss pipelines}}

 Prior works only focused on supervising the foreground (saliency) maps, whereas we supervised both the foreground (fg) and background (bg) maps. As seen from Table \ref{tab:bglosssupervision}, background supervision slightly improves performance over foreground supervision.

 \begin{table}[h!]
\centering
  \begin{tabular}{|c|c|c|}%|ccccc}
    \hline
      AGLRFE  & $F_{max}$ & MAE \\  %\multicolumn{5}{c}{SOD}\\
    \hline
     fg + bg & 0.917 & 0.029 \\
     fg & 0.911 & 0.031 \\
    \hline
  \end{tabular}
  % \end{adjustbox}
  \caption{Influence of background (bg) supervision on SODAWideNet++.}
  \label{tab:bglosssupervision}
 \end{table}
\vspace{-12mm}
\subsection{Reviewer 3 Comments}

We thank the reviewer for recommending exciting research directions, such as Implicit Neural Representation (INR) or the Mamba module for Salient Object Detection.
\\ \\
\textbf{\textit{Highlight how the proposed technique is important and what is key novelty comparing to existing approaches?}}

The proposed SODAWideNet++ is explicitly designed for SOD, unlike prior models that rely on ImageNet pre-trained backbones built primarily for image classification. This tailored design allows the entire network to be pre-trained simultaneously, allowing dense prediction based pre-training pipelines to be used for SOD and eliminating the classification-centric computationally expensive ImageNet pre-training.
The key contributions of our work are two folds. Firstly, we combine dilated convolutions and self-attention into a single unit whereas prior work use separate branches for convolutions and Attention. For example, PGNet uses a Swin branch and a ResNet branch as feature extractor. Secondly, we supervise both foreground (saliency) and background maps to generate better saliency predictions. Finally, we modify the COCO semantic segmentation dataset and use that to pre-train the proposed SODAWideNet++, illustrating the importance a dense pre-training pipeline instead fo the traditional ImageNet classification pre-training.

% Unlike traditional models that rely on ImageNet pre-trained backbones, SODAWideNet++ is explicitly designed for SOD, allowing for the pre-training of the entire network simultaneously. This eliminates computationally expensive ImageNet pre-training. Additionally, SOD-specific choices, such as capturing global features with minimal information loss, have resulted in a competitive yet lightweight model compared to other state-of-the-art models.

% Additionally, our model is lightweight compared to other state-of-the-art models, highlighting the advantages of domain-specific architectures, hence the importance of our proposed technique.

% % All the prior works in SOD are built on top of an ImageNet pre-trained backbone built particularly to perform well for Image Classification, a significantly distinct task from SOD. In contrast, we concentrate on creating a network made of components essential for a dense prediction task like SOD. This reduces reliance on ImageNet pre-training, which is very expensive and unfeasible with limited computing power. 

% The proposed Attention Guided Long Range Feature Extraction (AGLRFE) combines large dilated convolutions and self-attention into a single streamlined module that extracts long-range features. This combination leverages convolution operations' inductive biases and self-attention's input dependency to effectively identify salient objects of various sizes. For example, PGNet \cite{xie2022pyramid} uses separate convolution (ResNet) and attention (Swin) networks. Additionally, we supervise both foreground and background predictions. This dual supervision ensures the model generates more precise saliency maps by accurately distinguishing between salient objects and background regions. The influence of adding background supervision can be seen in Table \ref{tab:bglosssupervision}.
% Also, the proposed module, Attention Guided Long Range Feature Extraction (AGLRFE), combines large dilated convolutions and self-attention into a single streamlined module that extracts long-range features. This combination leverages convolution operations' inductive biases and self-attention's input dependency to effectively identify salient objects of various sizes. For example, PGNet \cite{xie2022pyramid} uses separate convolution (ResNet) and attention (Swin) networks. Additionally, we supervise both foreground and background predictions. This dual supervision ensures the model generates more precise saliency maps by accurately distinguishing between salient objects and background regions. The influence of adding background supervision can be seen in Table \ref{tab:bglosssupervision}.

\textbf{\textit{How is the generalization ability of this work? Especially in scenes with complex backgrounds or with multiple salient objects.}}

% SODAWideNet++'s architecture, combining dilated convolutions and self-attention, is well-suited to handle varied scenes and conditions, enabling it to capture local and global features effectively. This design makes the model robust in detecting salient objects, even in complex backgrounds or when multiple objects are present. Its competitive performance on several datasets, achieving high scores in F-measure (Fmax), Mean Absolute Error (MAE), and S-measure (Sm), further demonstrates its robustness. 

Visual results confirm that SODAWideNet++ can accurately detect salient objects in challenging scenarios, including images with large foreground objects (figure 4 rows one \& four), multiple objects (figure 4 row two), and complex backgrounds (figure 4 row three), showcasing its strong generalization ability across diverse visual conditions. Furthermore, its competitive performance on several datasets, as seen in Table 1, achieving high scores in F-measure ($F_{max}$), Mean Absolute Error (MAE), and S-measure ($S_{m}$), demonstrates its robustness.
\\ \\
\textbf{\textit{Can this model be further extended and applied to 360 VR images or videos? Even in multimodal situations, such as audio-visual saliency detection?}}

Although not designed for 360 VR, we believe our model is adaptable and can be extended to deal with the more complex field of view and spatial relationships of VR data. We also believe extra modalities such as audio, can enhance the model's performance in multimodal (audio-visual) saliency detection tasks.

% The model's ability to capture long-range dependencies and local features using AGLRFE and ALPM modules makes it adaptable to the unique challenges of 360 VR content, where the field of view and spatial relationships are more complex. Additionally, extra modalities, such as audio, could enhance the model's performance in multimodal saliency detection tasks. The self-attention mechanisms used in SODAWideNet++ can be extended to process and integrate features from multiple modalities, leveraging audio cues to improve visual saliency detection.

% Additionally, all the prior works in SOD are built on top of an ImageNet pre-trained backbone built particularly to perform well for Image Classification, a significantly distinct task from SOD. In contrast, we concentrate on creating a network made of components essential for a dense prediction task like SOD. This reduces reliance on ImageNet pre-training, which is very expensive and unfeasible with limited computing power.

% Also, simultaneously supervising the foreground and background is novel and adds an extra penalty to the model for inaccurate predictions.

% Yes, in future work, we will try to utilize Implicit Neural Representations and Mamba for SOD.

% The proposed SODAWideNet++ performs better on various datasets with complex backgrounds (DUT-OMRON, HKU-IS, and ECSSD) and images with multiple objects (PASCAL-S).
